Reassembly Codes for the Chop-and-Shuffle Channel

We study the problem of retrieving data from a channel that breaks the input sequence into a set of unordered fragments of random lengths, which we refer to as the chop-and-shuffle channel. The length of each fragment follows a geometric distribution. We propose nested Varshamov-Tenengolts (VT) codes to recover the data. We evaluate the error rate and the complexity of our scheme numerically. Our results show that the decoding error decreases as the input length increases, and our method has a significantly lower complexity than the baseline brute-force approach. We also propose a new construction for VT codes, quantify the maximum number of the required parity bits, and show that our approach requires fewer parity bits compared to known results.

==> sections/Appendices.tex <==
\section{Proof of theorem~\ref{theorem_length_parity}}
\label{appndx:thm_length_parity}

% {\color{red} repeat the theorem here. It is always nice to have the statement of the theorem, lemma, etc with their proof. Do this wherever needed.}


\begin{reptheorem}{theorem_length_parity}
Given any data-bit sequence of length $n_d$, it is possible to construct a VT code as defined in (\ref{eq_VT_def}) of length $n$ with residue $0 \leq r \leq n$ where $n = n_d + p$ for $p=\Big\lceil\frac{1+\sqrt{1+8n_d}}{2}\Big\rceil$.
\end{reptheorem}

\begin{proof}
According to \eqref{eq:construct_x}, $\textbf{x}=[\textbf{d} \quad \textbf{p}]$ is the VT codeword where \textbf{d} and \textbf{p} represent the data bits with length $n_d$ and parity bits with length $p$, respectively. We will show later in Appendix~\ref{appndix:find_parity} that we set
\begin{align}
    \label{eq:residue_Delta_appndix}
    \sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}\equiv \delta, \mod (n+1),
\end{align}
as the residue of parity bits where $0\leq\delta\leq n$. Moreover, we know that $\frac{p(p+1)}{2}$ is the maximum value of $\sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}$, which happens if all parity bits are equal to 1. As a result, to generate $\delta$, we need
\begin{align}
\label{eq:min_p_quad}
& \frac{p(p+1)}{2}\geq n=n_d+p\\ \nonumber 
& p^2-p\geq2n_d
\end{align}

To solve the quadratic inequality in (\ref{eq:min_p_quad}), we need to find $p$ in the equality case. To do this, we derive the roots of the following quadratic equality
\begin{align}
\label{eq:equality_p}
& p^2-p-2n_d=0 \\ \nonumber
& p=\frac{1\pm \sqrt{1+8n_d}}{2} \rightarrow \left\{
                \begin{array}{ll}
                  p_1= \frac{1- \sqrt{1+8n_d}}{2}\\
                  p_2=\frac{1+ \sqrt{1+8n_d}}{2}
                \end{array}
            \right.
\end{align}
Table~\ref{table:parity_length} depicts how equality in (\ref{eq:equality_p}) changes to different inequalities based on different values of $p$. It shows, (\ref{eq:min_p_quad}) is feasible when $p\leq p_1$ or $p\geq p_2$. Additionally, since $p$ is non-negative integer number, $p\leq p_1$ is not acceptable. As a result, we use $p=\ceil{p_2}=\ceil{\frac{1+\sqrt{1+8n_d}}{2}}$ as the minimum integer number that satisfy $p\geq p_2$, and this completes the proof. 

\begin{table}[ht]
\caption{Sign of $p$ in different intervals}
\centering
\begin{tabular}{|c|c|c|}
\hline
 $p \leq p_1$ & $p_1<p<p_2$ & $p\geq p_2$\\[0.5ex]
\hline
$``+"$ & $``-"$  & $``+"$  \\

\hline
\end{tabular}
\label{table:parity_length}
\end{table}
\end{proof}

\section{Finding parity bits $\textbf{p}$}
\label{appndix:find_parity}
In this section, we demonstrate how to obtain parity bits $\textbf{p}$ with length $p=\ceil{\frac{1+\sqrt{1+8n_d}}{2}}$ to ensure that the codeword $\textbf{x}$ meets the desired residue $r$. To do this, we define $r^{\prime}$ as
\begin{align}
    \sum_{i=1}^{n_d}id_i\equiv r^{\prime} \mod (n+1),
\end{align}
where $d_i$ is the $\text{i}^{\mathrm{th}}$ element of $\textbf{d}$. Moreover, we know that $\textbf{d}$ represents the first $n_d$ elements of $\textbf{x}$. Therefore, we have,
\begin{align}
\label{eq:sum_residue}
\sum_{i=1}^{n}ix_i&=\sum_{i=1}^{n_d}ix_i+\sum_{i=n_d+1}^{n}ix_i \\ \nonumber
&=\beta(n+1)+r^{\prime}+\sum_{i=n_d+1}^{n}ix_i\\ \nonumber 
&\overset{(i^{\prime} \triangleq n+1-i)}{=}\beta(n+1)+r^{\prime}+\sum_{i^{\prime}=1}^{n-n_d}(n+1-i^{\prime})x_{n+1-i^{\prime}}\\ \nonumber
&= \underbrace{\beta(n+1)}_{a_1}+r^{\prime}+\underbrace{(n+1)\sum_{i^{\prime}=1}^{p}x_{n+1-i^{\prime}}}_{a_2}\\ \nonumber
&-\sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}.
\end{align}
Then, we use \eqref{eq:sum_residue} to calculate the residue. We know that the residues of $a_1$ and $a_2$ in \eqref{eq:sum_residue} equal to zero. As a result, we have,
\begin{align}
    \label{eq:residue_i_xi}
    \sum_{i=1}^{n}ix_i\equiv r^{\prime}-\delta, \mod (n+1),
\end{align}
where $\delta$ is equal to 
\begin{align}
    \label{eq:residue_Delta}
    \sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}\equiv \delta, \mod (n+1).
\end{align}
Here, \eqref{eq:residue_Delta} shows that by calculating the residue of codeword $\textbf{x}$ from the right-hand side (starting from the parity bits), $\delta$ represents the residue of parity bits string from the right-hand side. Therefore, to achieve the desired residue $r$, all we need is to create parity bits $\textbf{p}$ such that $\delta$ is equal to
\begin{equation}
\delta=\left\{
                \begin{array}{ll}
                  r^{\prime}-r \quad \quad \quad \quad \quad \quad ~r^{\prime}\geq r,\\
                  (n+1)-(r-r^{\prime}) \quad r^{\prime}< r.
                \end{array}
            \right.
\end{equation}


To derive parity bits $\textbf{p}$, we propose a four-step procedure as below: 

{\it Step 1 $\rightarrow$ Define $k=p-i^{\prime}+1$}: We use $k$ to show the position of parity bit which starts from left side of parity bits;

{\it Step 2 $\rightarrow$ Solve $pk-\frac{k(k-1)}{2}\leq \delta$:} We solve this inequality and obtain the largest non-negative integer value of $k$ as $k_{max}$. Here, it is essential to show that $pk-\frac{k(k-1)}{2}\leq \delta$ is feasible for $p\geq 1$. To do this, we have
\begin{align}
\label{eq:j_max_inequal}
& pk-\frac{k(k-1)}{2}\leq \delta \\ \nonumber
& pk-\frac{k(k-1)}{2}\leq \delta \overset{(a)}{\leq} \frac{p^2+p}{2} \\ \nonumber
& k^2-(2p+1)k+p^2+p\geq 0,
\end{align}
where $(a)$ holds true since the maximum value of $\delta$ is equal to $(p^2+p)/2$ when all bits of $\textbf{p}$ are equal to 1.
To solve the quadratic inequality in (\ref{eq:j_max_inequal}), we need to find $k$ in the equality case. More precisely, we derive the roots of the following quadratic equality
\begin{align}
\label{eq:j_max_equal}
& k^2-(2p+1)k+p^2+p=0 \\ \nonumber
& k=\frac{2p+1\pm 1}{2} \rightarrow \left\{
                \begin{array}{ll}
                  k_1= \frac{2p}{2}=p\\
                  k_2=\frac{2p+2}{2}=p+1.
                \end{array}
            \right.
\end{align}

Table~\ref{table:j_max} shows how different values of $k$ change the equality in (\ref{eq:j_max_equal}) to various inequalities.
\begin{table}[ht]
\caption{Sign of $k$ in different intervals}
\centering
\begin{tabular}{|c|c|c|}
\hline
 $k \leq k_1$ & $k_1<k<k_2$ & $k\geq k_2$\\[0.5ex]
\hline
$``+"$ & $``-"$  & $``+"$  \\

\hline
\end{tabular}
\label{table:j_max}
\end{table}

According to the results of table~\ref{table:j_max}, either $k_{max}\leq p$ or $k_{max}\geq p+1$ satisfies the inequality in (\ref{eq:j_max_inequal}). Moreover, we know $0\leq k_{max}\leq p$ and $k_{max}$ at most can be equal to $p$. As the result, it shows that always there is $0\leq k_{max}\leq p$, which satisfies the quadratic inequality in (\ref{eq:j_max_inequal}), and this proves that $pk-\frac{k(k-1)}{2}\leq \delta$ is feasible for $p\geq 1$. 


{\it Step 3 $\rightarrow$ Put all parity bits in $1\leq k \leq k_{max}$ equal to 1 when $k_{max}>0$:} In this step, we create an initial version of parity bits by placing one in the position(s) of $1\leq k \leq k_{max}$. Consequently, we have an initial parity bits such that $\sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}=pk_{max}-\frac{k_{max}(k_{max}-1)}{2}$;

{\it Step 4 $\rightarrow$ Place parity bit in position $b$ where $b \triangleq\delta-pk_{max}-\frac{k_{max}(k_{max}-1)}{2}$:} From {\it Step 3}, we know that
\begin{align}
\label{eq:p_k_max_less_delta}
    \sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}=pk_{max}-\frac{k_{max}(k_{max}-1)}{2}\leq \delta.
\end{align} 
Therefore, to convert the inequality to equality in \eqref{eq:p_k_max_less_delta}, we add $b=\delta-pk_{max}-\frac{k_{max}(k_{max}-1)}{2}$ to $\sum_{i^{\prime}=1}^{p}i^{\prime}x_{n+1-i^{\prime}}$ in \eqref{eq:p_k_max_less_delta}. To do this, we put 1 in the position of $b$.


\section{Complexity of finding parity bits $\textbf{p}$}
\label{appndix:complexity_parity}

In this appendix, we describe the complexity of our strategy to find parity bits. To explain the details, we divide the complexity into the following three parts:

{\it (i) $\sum_{i=1}^{n} ix_i$:}

Here, we need to perform $(n-1)$ additions to get $\sum_{i=1}^{n} ix_i$. We note that we do not need multiplications as $x_i \in \{0,1\}$, which simply means add or do not add $i$. Furthermore, each addition is a constant-time operation. Thus, $\mathcal{O}(n)$ is the complexity of $\sum_{i=1}^{n} ix_i$;

{\it (ii) Mod function:}

The author in \cite{shoup2009computational}, %-Theorem 3.3,
shows that the computing complexity of mod function of $r\equiv \sum_{i=1}^{n} ix_i ~~\text{mod}(n+1)$ is $\mathcal{O}(\text{length}(n+1) \times \text{length}(q))$ where $q$ satisfies \begin{align}
   \sum_{i=1}^{n} ix_i=q(n+1)+r, 
\end{align}
and $\text{length}(z)=\lfloor\log_2(z)\rfloor+1$ describes the length of number $z$ in binary domain where $\lfloor.\rfloor$ is the floor function. 
We know that $q\leq \frac{n}{2}$ because $\sum_{i=1}^{n} ix_i\leq \frac{n(n+1)}{2}$. Hence, the computing complexity of mod function is $\mathcal{O}(\text{length}(n+1)\times\text{length}(\frac{n}{2}))= \mathcal{O}(\Big[\lfloor\log_2(n+1)\rfloor+1 \Big] \times \Big[\lfloor\log_2\frac{n}{2}\rfloor+1 \Big])$;

{\it (iii) Solving quadratic inequality:}

In \cite{kim1994polynomial}, the authors explain that the complexity of finding the roots of a quadratic polynomial with $\gamma$-error is equal to 
\begin{align}
    \mathcal{O}(2(\log_{10}2)^2|\log_{10}\gamma|+4(\log_{10}2)^2).
\end{align}
We note that since all calculations are done in the binary domain, we need to take into account the complexity of converting the root of the quadratic equation into the binary domain, which is given as
\begin{align}
    \mathcal{O}(\lfloor \log_2 k_{max} \rfloor +1)\overset{(a)}{\leq}\mathcal{O}(\lfloor \log_2 p \rfloor +1)\overset{(b)}{<}\mathcal{O}(\lfloor \log_2 n \rfloor +1),
\end{align}
where $(a)$ and $(b)$ hold true since $k_{max}\leq p<n$. As a result, the overall complexity of finding the root of the quadratic equation equals to $\mathcal{O}(\lfloor \log_2 n \rfloor +1)$.

According to the above results, we conclude that the complexity of our encoding method is also linear (i.e., $\mathcal{O}(n)$), similar to Sloane's approach in \cite{sloane2002single}. 

\section{Proof of theorem~\ref{theorem:encoding_rate}}
\label{appndix_proof_encoding_rate}

\begin{reptheorem}
{theorem:encoding_rate}
Given that $n_d=m^{(\ell-1)}d_{sec}$ is the length of data bits $\textbf{d}$ and for $d_{sec}\geq 36$, the encoding rate of the $\ell$-layered nested VT code is bounded by 
\begin{align}
R^-<R<R^+,
\end{align}
where 
\begin{align}
    R^-=\frac{m^{\ell-1}d_{sec}}{\Big(m^{(\frac{\ell-1}{2})}\sqrt{d_{sec}}+\frac{\sqrt{2.5}}{2}\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1}\Big)^2},
\end{align}
and the upper bound, $R^+$, is equal to
\begin{align}
    R^+=\frac{2m^{\ell-1}d_{sec}}{\Big(m^{(\frac{\ell-1}{2})}\sqrt{2d_{sec}}+\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1}\Big)^2}.
\end{align}
\end{reptheorem}

\begin{proof}
Our nested VT code with $\ell$ layers converts the input data-bits $\textbf{d}$ with length $m^{(\ell-1)}d_{sec}$ to the codeword $\textbf{x}$ with length $n$. Hence, the encoding rate is
\begin{align}
\label{eq_R_general}
    R=\frac{m^{(\ell-1)}d_{sec}}{n},
\end{align}

To obtain the lower and upper bounds on $R$, we need to find the lower and upper bounds of $n$. Therefore, we divide the proof into two parts:

$\bullet~\textbf{Lower bound on n}$

According to Theorem~\ref{theorem_length_parity}, the length of each codeword in the first layer is equal to
\begin{align}
\label{tilda_n_1}
    \Tilde{n}_1=d_{sec}+\Bigg\lceil\frac{1+\sqrt{1+8d_{sec}}}{2}\Bigg\rceil,
\end{align}
Next, we have
\begin{align}
\label{eq:lower_tilda_n_1}
  \Tilde{n}_1&\overset{(a)}{\geq}d_{sec}+\frac{1+\sqrt{1+8d_{sec}}}{2}\\ \nonumber
  &>d_{sec}+\frac{1+\sqrt{8d_{sec}}}{2}=\frac{(\sqrt{2d_{sec}}+1)^2}{2},
\end{align}
where $(a)$ is correct because $\ceil{u}\geq u$ for any real number $u$. Then, we define $\Tilde{d}_{sec}\triangleq\sqrt{2d_{sec}}$ and rewrite \eqref{eq:lower_tilda_n_1} as
\begin{align}
   \Tilde{n}_1>\frac{(\Tilde{d}_{sec}+1)^2}{2}.
\end{align}
Moreover, $\Tilde{n}_2$ contains $m$ different sections of $\Tilde{n}_1$, which means
\begin{align}
\label{eq:n2_tilde}
   \Tilde{n}_2=m\Tilde{n}_1+\Bigg\lceil\frac{1+\sqrt{1+8m\Tilde{n}_1}}{2}\Bigg\rceil. 
\end{align}
Similar to \eqref{eq:lower_tilda_n_1}, we have 
\begin{align}
    \Tilde{n}_2&>\frac{(\sqrt{2m\Tilde{n}_1}+1)^2}{2}=\frac{(\sqrt{m}(\Tilde{d}_{sec}+1)+1)^2}{2}.
\end{align}
Then, following the same rule, we can show that
\begin{align}
\label{eq_lower_n_L}
   &\Tilde{n}_{\ell}
   \\ \nonumber
   &>\frac{(\overbrace{\sqrt{m}(\sqrt{m} \ldots \sqrt{m} }^{\ell-1~ \text{coefficients}}(\Tilde{d}_{sec}+1)\overbrace{+1)+1)\ldots )+1}^{\ell-1~ \text{coefficients}})^2}{2}\\ \nonumber
   &=\frac{(m^{(\frac{\ell-1}{2})}\Tilde{d}_{sec}+m^{(\frac{\ell-1}{2})}+m^{(\frac{\ell-2}{2})}+\ldots+\sqrt{m}+1)^2}{2}\\ \nonumber
   &=\frac{1}{2}(m^{(\frac{\ell-1}{2})}\Tilde{d}_{sec}+\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1})^2\\ \nonumber
   &=\frac{1}{2}(m^{(\frac{\ell-1}{2})}\sqrt{2d_{sec}}+\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1})^2,
\end{align}
which represents a lower bound on $n$ since the nested VT code in $\ell^{\mathrm{th}}$ layer includes only one section (i.e., $n=\Tilde{n}_{\ell}$).

$\bullet~\textbf{Upper bound on n}$

To derive an upper bound on $n$, we have
\begin{align}
\label{simp_tilda_n_1}
  \Tilde{n}_1&\overset{(b)}{<}(d_{sec}+1)+\frac{1+\sqrt{1+8d_{sec}}}{2}\\ \nonumber
  &<(d_{sec}+1)+0.5+\sqrt{2(d_{sec}+1)}\\ \nonumber
  &=(\sqrt{d_{sec}+1}+\frac{\sqrt{2}}{2})^2\overset{(c)}{<}(\sqrt{d_{sec}}+\frac{\sqrt{2.5}}{2})^2,
\end{align}
where $(b)$ holds true since $\ceil{u}<u+1$ for any real number $u$. Then, to show for which range of $ d_ {sec}$, $ (c)$ is true, we extend the inequality in \eqref{simp_tilda_n_1} as
\begin{align}
\label{eq:dsec_ineq_1}
    d_{sec}+\frac{3}{2}+\sqrt{2(d_{sec}+1)}&<d_{sec}+0.625+\sqrt{2.5d_{sec}}\\ \nonumber
    0.875+\sqrt{2(d_{sec}+1)}&<\sqrt{2.5d_{sec}},
\end{align}
where both sides of \eqref{eq:dsec_ineq_1} are positive numbers, and doubling them does not change the inequality. Thus, we have
\begin{align}
\label{eq:dsec_ineq_2}
    (0.875+\sqrt{2(d_{sec}+1)})^2&<(\sqrt{2.5d_{sec}})^2\\ \nonumber
    2.47\sqrt{(d_{sec}+1)}&<0.5d_{sec}-2.766 \\ \nonumber
    (2.47\sqrt{(d_{sec}+1)})^2&\overset{(d)}{<}(0.5d_{sec}-2.766)^2 \\ \nonumber
    -d_{sec}^2+35.464d_{sec}-6.2&<0.
\end{align}
where $(d)$ happens because two sides of inequality are positive numbers. Then, by solving \eqref{eq:dsec_ineq_2}, we obtain that $d_{sec}>35.288$, which means that condition $(c)$ in \eqref{simp_tilda_n_1} holds true if $d_{sec}\geq 36$. 

Finally, following the same steps in deriving the lower bound of $n$ leads to
\begin{align}
\label{eq_upper_n_L}
   \Tilde{n}_{\ell}
   <(m^{(\frac{\ell-1}{2})}\sqrt{d_{sec}}+\frac{\sqrt{2.5}}{2}\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1})^2.
\end{align}
Here, we use \eqref{eq_R_general}, \eqref{eq_lower_n_L}, and \eqref{eq_upper_n_L} to conclude that
\begin{align}
R^{-}<R<R^+,
\end{align}
where 
\begin{align}
    R^-=\frac{m^{\ell-1}d_{sec}}{\Big(m^{(\frac{\ell-1}{2})}\sqrt{d_{sec}}+\frac{\sqrt{2.5}}{2}\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1}\Big)^2},
\end{align}
and
\begin{align}
    R^+=\frac{2m^{\ell-1}d_{sec}}{\Big(m^{(\frac{\ell-1}{2})}\sqrt{2d_{sec}}+\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1}\Big)^2},
\end{align}
and this completes the proof.
\end{proof}






==> sections/Introduction.tex <==
%{\color{brown}
Recently DNA-based storage has emerged as a promising technology for durable data storage with enormous information density. Several works \cite{church2012next,goldman2013towards,grass2015robust,yazdi2015rewritable,erlich2017dna,organick2018random} have presented DNA-based storage prototypes, which are capable of storing up to 200 Megabytes of data.

DNA contains four nucleotides (Adenine, Cytosine, Guanine, and Thymine), and data can be mapped from the binary domain into the nucleotide domain for storage purposes. However, the DNA strings are exposed to breaks during writing (synthesizing) and reading (sequencing) procedures. During the synthesis process, data is
written onto DNA molecules and stored in a solution where molecules
in the solution are subject to random breaks. As for reading/sequencing, there are two standard methods: (1) {\it Shotgun sequencing} that provides a cost-efficient, high-throughput platform and samples a long DNA molecule with a large number of
short reads. In particular, this method reads the data from random locations of the DNA sequences in a DNA pool
in a parallel fashion~\cite{motahari2013information,yazdi2015rewritable,bornholt2016dna}. However, shotgun sequencing does not create a long sequence, which has potentials for higher density storage and faster reading process; (2) {\it Nanopore sequencing} that enables reading of several thousand bases at a time by moving the DNA string through a small pore with radius in the order of a nanometer~\cite{branton2010potential,bleidorn2016third,jain2016oxford}. However, Nanopore sequencing creates variable-length sequences and increases the error
rate and cost compared to shotgun sequencing. We note that the two common sequencing methods create unordered DNA fragments with fixed or variable lengths, which require reassembly and result in the shuffling channel~\cite{shomorony2020communicating};

Motivated by the above results, in this paper, we consider a chop-and-shuffle channel where the input is a length-$n$ binary data bits (which would be easy to extend to nucleotide domain) that is chopped into a random number, $M$, fragments with lengths $L_1, L_2, \ldots, L_M$ where $L_j, 1\leq j \leq M$ is a random variable with Geometric$(p_n)$ distribution. Here, the channel output is an unordered set of variable-length elements that are shuffled.

The capacity of a chop-and-shuffle channel %(refer as {\it torn-paper channel}) \iscomment{may be better not to mention the name torn-paper channel} 
with variable-length fragments is characterized in~\cite{shomorony2020communicating,TornPaperCoding} as
\begin{align}
    \label{eq:capacity}
    C=e^{-\alpha},
\end{align}
where $\alpha = \lim_{n \rightarrow \infty}{p_n \log_2(n)}$, and \cite{shomorony2020communicating,TornPaperCoding} achieve the capacity via random coding. However, random coding is not a practical solution, and in~\cite{TornPaperCoding} a constructive code is also presented but the achievable rates fall short of the capacity. 


The main contributions in this paper are as follows:

\begin{itemize}
    \item We devise layered Varshamov-Tenengolts (VT) codes, called ``Nested VT codes,'' to recover the input data from the broken fragments of a chop-and-shuffle channel; %We also apply an erasure code, preceded the nested VT code, to capture the impact of the fact that too short fragments can fit many different places 
    %{\color{red} Sajjad, you told me this is in fact not the case! remove this last sentence. Remove similar statements throughout the paper. The addition of the erasure code is a minor issue anyway.};
    \item We focus on scenarios where the channel capacity $C \leq 1$ (i.e., $0 \leq \alpha \leq 1$) and determine the achievable rates of the nested VT codes numerically;  %{\color{red} remove the next sentence. This part summarizes your key contributions and having a limited time for simulation isn't one.} Furthermore, we {\color{brown} consider a limited timeframe to run the decoding algorithm and} show that the decoding error decreases as $n$ increases;
    \item We study the complexity of our reassembly algorithm in terms of the number of required iterations to recover the input data and illustrate that our method significantly reduces the computational complexity compared to the brute-force approach (which checks all possible permutations);
    \item Finally, we also present a new construction for individual VT codewords with linear complexity that needs fewer parity bits compared to prior results.
\end{itemize}
%}



\subsection{Related work}
\label{subsec:related_work}

%{\color{brown}
Rapid advances in DNA-based storage with today's technology attract a significant amount of research attention from an information-theoretic perspective where DNA-based storage acts as a communication channel~\cite{kiah2016codes,yazdi2015rewritable,erlich2017dna,lenz2020achieving,shomorony2019capacity,lenz2019coding}. Among these, \cite{shomorony2019capacity,lenz2019coding} use coding over a set of short sequences that are randomly sequenced and then shuffled in an unordered fashion. In particular, \cite{shomorony2021dna} studies a storage channel assuming each random sequence is read precisely once, and substitution noise is the only source of error. Then, \cite{lenz2019coding} proposes some error-correcting codes under different scenarios suitable for insertions, deletions, and substitution errors. We note that the above works examine cases with sequences of equal length, while in this paper, we focus on variable-length fragments. 

Moreover, extracting data from a set of its subsequences has been studied in several works \cite{motahari2013information,bresler2013optimal} %\iscomment{these papers are not about DNA storage, they are about assembling real genomes}
where the data is retrieved from real genome sequences. More precisely, \cite{motahari2013information} shows the minimum number of required reads for
reliable reconstruction and  \cite{bresler2013optimal} demonstrates an optimal assembly algorithm for complete reconstruction. Despite these works assume that the observed sequences overlap, in this paper, we propose an encoding/decoding approach that fits non-overlapping sequences. 

As we described above, the capacity of a chop-and-shuffle channel with variable-length fragments is determined and achieved using random coding in~\cite{shomorony2020communicating}.
%} %\iscomment{it's a bit weird to mention this since $p_n$ and $n$ are not defined}. 
Then, \cite{TornPaperCoding} proposes an interleaved-pilot scheme based on de Bruijn sequences to encode and decode the data bits. In particular, \cite{TornPaperCoding} provides a lower-bound on the achievable rate by considering a parity string $\textbf{p}$ with length $n/\zeta$ where $\zeta\geq 2$ is a positive integer and $n$ is the length of encoded bits. Then, it shows that if the length of $j^{\mathrm{th}}$ fragment, $L_j, 1\leq j\leq M$, contains at least $L_j/\zeta$ parity bits in it, the proposed approach allows the decoder to recover the data bits uniquely for long enough $L_j$. However, there is a big gap between the achievable rate of the approach in \cite{TornPaperCoding} and the capacity. As a result, in this paper, we focus on an efficient code based on VT codes that provides higher achievable rate, compared to \cite{TornPaperCoding}. 

Furthermore, in~\cite{nassirpour2020embedded}, we also use the chop-and-shuffle channel to model a DNA-based storage channel where DNA breaking is the main source of error. Then, we present a practical encoding/decoding mechanism based on an embedded structure of VT codes to recover data from DNA fragments (outputs of the chop-and-shuffle channel). However, the results of~\cite{nassirpour2020embedded} are limited to $\alpha =0$ (i.e., capacity is $1$) and do not generalize to $0<\alpha<1$. %This means that if the channel breaks at higher rates ($\alpha>0$), the embedded VT code fails to reconstruct the data bits. While 
In this manuscript, we present a new solution, Nested VT codes, for $0<\alpha<1$. %concentrate on the scenarios with a higher number of broken fragments, compared to \cite{nassirpour2020embedded}, where $0 \leq \alpha \leq 1$ and 
%concentrate on the scenarios with a higher number of broken fragments, compared to \cite{nassirpour2020embedded} where.
%\iscomment{this paragraph is confusing, and the last sentence seems incomplete. Does [21] consider $\alpha = 0$ or $0 \leq \alpha \leq 1$?}

% \iscomment{I think the introduction needs to be more clear about what the problem is and what the previous approaches are. This is not easy to follow if you are not familiar with [5], [6] and [7].}

% \sncomment{I have updated the Intro. Please check the details.}


\subsection{Notations}
\label{subsec:notation}

Table~\ref{table:param} summarizes the notations we use in this paper.

\begin{table}[ht]
\caption{Parameters used in this paper.}
\centering
\begin{tabular}{|c|l|}
\hline

%Parameters  \\[0.5ex]
Parameter & \hspace{1.2in} Description \\
\hline \hline%\hline
$\textbf{d}$ & Input data bits. \\
$n_d$ & Length of $\textbf{d}$.\\
$d_{sec}$  & Length of one section of $\textbf{d}$.\\
$\textbf{x}$ & Nested VT codeword. \\
$\ell$ & Number of layers in $\textbf{x}$.\\
$n$ & Length of $\textbf{x}$.\\
$\textbf{d}^{(l)}_i$ & $i^{\mathrm{th}}$ section of data bits in $l^{\mathrm{th}}$ layer.\\
$\textbf{x}^{(l)}_i$ & VT codeword corresponding to $\textbf{d}^{(l)}_i$.\\
$r^{(l)}_i$ & Residue of $\textbf{x}^{(l)}_i$.\\
$\mathbf{y}_j$ & $j^{\mathrm{th}}$ broken fragment.\\
$L_j$ & Length of $\mathbf{y}_j$.\\
$S(\textbf{x})$ & Set of broken fragments.   \\
$\hat{\textbf{x}}$ & Estimated version of $\textbf{x}$.\\
$\hat{\textbf{x}}^{(l)}_i$ & Estimated version of $\textbf{x}^{(l)}_i$.\\
$\hat{\textbf{d}}^{(l)}_i$ & Estimated version of $\textbf{d}^{(l)}_i$.\\
$\hat{\textbf{d}}$ & A guess of data bits ${\textbf{d}}$.\\
$M$ & Number of fragments created by the chop-and-shuffle\\
& channel.\\
m & Number of VT codewords in each layer that create a new\\
& data section in the next layer.\\[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:param}
\vspace{-2mm}
\end{table} 

%{\color{brown}
\subsection{Outline}

The rest of the paper is organized as follows. In Section~\ref{Section:Problem}, we formulate
the problem. In Section~\ref{Section:Main}, we present the main results of the paper, which include our layered design for VT codes, referred to as nested VT code, a new construction for a single VT code, and the encoding rate of the nested VT code. Then, we provide details on why our encoding/decoding scheme contains an erasure code and the nested VT code in Section~\ref{Section:erasure_nested}. In Sections~\ref{Section:Nested_encoder} and \ref{Section:Nested_decoder}, we explain our proposed encoder and decoder, respectively. We show our results via a numerical example in Section~\ref{Section:simulations}, and section~\ref{Section:conclusion} concludes the paper.
%}

==> sections/Section2_problem_setting.tex <==
Our goal is to devise practical codes for the chop-and-shuffle
channel (CSC) depicted in Fig.~\ref{Fig:channel_model} to reliably communicate an input message $W$ chosen uniformly at random from $\{1,2,...,2^{nR}\}$. In particular, we wish to devise constructive codes to map the input message to a length-$n$ binary codeword $\textbf{x} \in \{0,1\}^n$. 

\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=6.5, width=0.65\linewidth]{images/channel_model.png}
  \caption{\it The chop-and-shuffle channel breaks codeword $\textbf{x}$ into $M$ variable-length fragments and then shuffles them where these unordered $M$ fragments are the input of the decoder.\label{Fig:channel_model}}
\end{figure}

%{\color{red} Sajjad, where have you defined the rate? achievable rate? capacity? You should say the input is a message $W$ uniformly chosen at random from $\{ 1,2, \ldots, 2^{nR}\}$, which is then encoded as $\textbf{x} \in \{0,1\}^n$. Follow one of my papers, like Torn-Paper Coding, you need to define the error probability based on which you can define the achievable rate and then the capacity. Also, later you can say $W$ is represented by the initial bit sequence. The figure is the problem of communication over the chop-and-shuffle channel not the channel itself. Encoder and decoder are not part of the channel!}

%Fig.~\ref{Fig:channel_model} depicts the chop-and-shuffling channel where $\textbf{d}$ is the input data bits. Then, $\textbf{d}$ is converted to the encoded codeword $\textbf{x} \in \{0,1\}^n$ with length $n$. 
The chop-and-shuffle channel can be described as follows. The channel first breaks $\textbf{x}$ into $M$ random-length fragments (where $1\le M\le n$ is random itself), and then shuffles these fragments resulting in an unordered set of output fragments. We use $\mathbf{y}_j$, $L_j$, and $S(\textbf{x})=\{\mathbf{y}_1,\mathbf{y}_2,\ldots,\mathbf{y}_M\}$ to denote the $j^{\mathrm{th}}$ output fragment, its corresponding length, and the set of all fragments (i.e., channel output), respectively. We note that $M=1$ implies that the input sequence has gone through the channel perfectly (i.e., no error). 

We assume $L_j$, $1 \leq j \leq (M-1)$, are independently and identically distributed (i.i.d.) random variables having a Geometric distribution as:
\begin{align}
    \label{eq:geometric_ditrb}
    L_j\thicksim \mathrm{Geom}(p_n), \quad 1 \leq j \leq (M-1),
\end{align}
where $0 \leq p_n \leq 1$ captures how frequently codeword $\textbf{x}$ is broken. Since the total length of the fragments should be equal to the length of codeword $\textbf{x}$, we have
\begin{align}
\label{eq:total_length_broken}
    \sum_{j=1}^{M}L_{j}=n,
\end{align}
where the length of the last fragment is determined based on other fragments as
\begin{align}
L_M = n - \sum_{j=1}^{M-1}{L_j}.
\label{length_final_fragment}
\end{align}

Finally, the decoder knows $p_n$ and uses $S(\mathbf{x})$ to find an estimate $\hat{W}$ of the input message $W$. An error occurs if $\hat{W}\neq W$, and the average probability of
decoding error is equal to
\begin{align}
    e_n=\mathbb{E}[\Pr\{\hat{W}\neq W\}],
\end{align}
where the expectation is over the random choice of message $W$ and the randomness of the CSC. 
We say that rate $R$ is achievable if there exist encoders and decoders such that $e_n \rightarrow 0$ as $n \rightarrow \infty$. Then, the capacity $C$ is defined as the supremum of all achievable rates.

% We define $\mathcal{C}$ as a set of $2^{nR}$ binary codewords with rate $R$ and length $n$, and say that the rate $R$ is achievable if there exist $\mathcal{C}_n \subset \mathcal{C}$, which includes length-$n$ codewords and results in $e_n \rightarrow 0$ as $n \rightarrow \infty$. Moreover, the capacity $C$ is defined as the supremum of all achievable rates.

% Later, in Section~\ref{Section:Nested_encoder}, $W$ is represented by the initial bit sequence.

% Finally, in the decoding stage, we are looking for a permutation, $\hat{\textbf{x}}$, as the estimation of the codeword that reassembles the data fragments correctly. 

%In this paper, we propose a layered version of Varshamov-Tenengolts (VT) codes suitable for retrieving data bits in the chop-and-shuffle channel. In the next section, we present the main results of this paper.

%encode/decode the data bits, and our decoder wishes to obtain a permutation that satisfies the VT conditions. Later, we demonstrate what the VT conditions mean. 

% Notice that the chop-and-shuffle channel creates $M$ different fragments, consequently, $M!$ possible permutations, and finding an appropriate permutation among these $M!$ choices makes the decoding part more challenging. In the next section, we present the main results of this paper.

==> sections/Section3_main_results.tex <==
% {\color{red} (1) ``We propose a new nested structure for Varshamov-Tenengolts codes.'' when you say modified, it implies it has the same form but with some changes. (2) there are no ``errors'' in chop-and-shuffle channel! Also, in general, we say ``correct erros'' not combat them. (3) how is paragraph 1 connected to paragraph 2? It is sudden and irrelevant jump.}

In this section, we propose a new layered design for Varshamov-Tenengolts codes that we refer to as ``Nested VT codes,'' which enable recovering data from the output fragments of the chop-and-shuffle channel. In the process, we present a new construction for an individual VT code that suits our designs. Finally, we describe the encoding %achievable 
rate of our scheme. Below, we explain the details.

\subsection{Nested VT code}
We first introduce the nested VT code for the chop-and-shuffle channel. VT codes were initially introduced for asymmetric Z-channels in~\cite{varshamov1965codes} as given below.
\begin{definition}
\label{def_VT}
\cite{sloane2002single} For $0\leq r \leq n$, the Varshamov-Tenengolts (VT) code $\textbf{x}$ is a binary encoded string with length $n$ satisfying
\begin{equation}
\label{eq_VT_def}
\sum_{i=1}^{n}ix_i\equiv r \mod (n+1)
\end{equation}
where $x_i$ is the $i^{\mathrm{th}}$ element of $\textbf{x}$ and the sum is evaluated as an ordinary  integer summation, and $r$ is referred to as the residue.

%\sncomment{I just used the definition of VT code in \cite{sloane2002single}, but it's redundant because all integers are rational. }
\end{definition}
In~\cite{levenshtein1966binary}, it was shown that VT codes can correct single deletions in the data bits, and in fact, VT codes have been used in deletion channels extensively~\cite{helberg2002multiple,abdel2011helberg,abroshan2019coding,mappouras2019greenflag}. %{\color{red} add more citations, look up Henry Pfister's work on deletion channels}

We concatenate and stack individual VT codes with a fixed residue (e.g., $r=0$) %different residues %\iscomment{maybe mention that $r$ is called the residue} 
in several layers to outline our nested VT code. %\sncomment{As we describe later, we use $r_i^{(l)}$ to show the residue of the $i^{\mathrm{th}}$ VT codeword in layer $1 \leq l \leq \ell$. I think since we don't use $r$ to describe different residues in different layers, mentioning $r$ here can be confusing to the reader.} 
We use superscript $(l), 1 \leq l \leq \ell$ to denote the parameters in $l^{\mathrm{th}}$ layer of the nested VT code. 

\textbf{Nested VT encoder:} We design our $\ell$-layered encoder to convert the input data bits $\textbf{d}$ with length $n_d$ to codeword $\textbf{x}$ with length $n$. More precisely, our nested VT encoder applies the following steps to create $\textbf{x}$: 
\begin{enumerate}

\item It breaks $\textbf{d}$ into $m^{\ell-1}$ small data sections with length $d_{sec}$ where $m$ represents the number of sections that combine together in each layer. Next, it encodes the $i^{\mathrm{th}}$ data section, $\textbf{d}_{i}^{(1)}, 1\leq i \leq m^{\ell-1}$, to $\textbf{x}_i^{(1)}$, the $i^{\mathrm{th}}$ VT codeword in layer 1 with residue $r_i^{(1)}=0$;

\item Going from layer $l$ to $l+1$, $1 \leq l < \ell$, $m$ VT codewords in layer $l$ are concatenated to form a new data section in for layer $l+1$ ($\mathbf{\textbf{d}}^{(l+1)}_{i}=[\mathbf{\textbf{x}}^{(l)}_i$, $\mathbf{\textbf{x}}^{(l)}_{i+1}$,$\ldots$, $\mathbf{\textbf{x}}^{(l)}_{i+m-1}]$), and then encoded as a new VT code. This reduces the number of sections by a factor of $m$. Finally, the $\ell^{\mathrm{th}}$ layer includes only one VT codeword.

%\iscomment{how do you combine $m$ VT codewords to form a new one? Figure 2 helps understand, but maybe this should be a bit more concrete}

%\sncomment{Specifically, we create $\mathbf{\textbf{d}}^{(l+1)}_{i}=[\mathbf{\textbf{x}}^{(l)}_i$, $\mathbf{\textbf{x}}^{(l)}_{i+1}$,$\ldots$, $\mathbf{\textbf{x}}^{(l)}_{i+m-1}]$ as the $i^{\mathrm{th}}$ data section in layer $l+1$, and then we apply VT code on $\mathbf{\textbf{d}}^{(l+1)}_{i}$. This reduces} the number of sections by a factor of $m$. Finally, the $\ell^{\mathrm{th}}$ layer includes only one VT codeword.

%   In the second layer, every $m$ VT codeword sections of the first layer merge together and create a new data section of the second layer. Thus, in this layer, we have $m^{\ell-2}$ different data sections. Then, similar to the first layer, our encoder converts the data bits sections to the codeword sections using corresponding residues;

% \item The encoder follows the procedure described in step (b) in the rest of the encoding layers. Finally, the $\ell^{\text{th}}$ layer includes only one VT codeword section, which we call $\textbf{x}$, the output of the nested VT code.  

\end{enumerate}

\begin{figure}[!ht]
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/nested-vt-encoder.png}
  \caption{\it Nested VT encoder with four layers and $m=2$.\label{Fig:nested_VT_encoder_pattern}}
\end{figure}

Fig.~\ref{Fig:nested_VT_encoder_pattern} depicts an example of the nested VT encoder with $\ell=4$ and $m=2$.  We will explain the technical details of the nested VT encoder in Section \ref{Section:Nested_encoder}.

We note that $\ell$ and $m$ are design parameters that determine the attained rate and the average error. We will derive upper and lower bounds on the rate associated with the nested VT code in Theorem~\ref{theorem:encoding_rate}. 

\textbf{Nested VT decoder:} The output of the chop-and-shuffle channel is $M$ different fragments with variable lengths. Here, our goal is to create a combination of these fragments that satisfies all VT conditions in different layers. We name this combination $\hat{\textbf{x}}$ as an estimated version of $\textbf{x}$, and then remove the parity bits from $\hat{\textbf{x}}$ to recover $\hat{\textbf{d}}$. 

We provide a high-level overview here and defer the technical details to Section~\ref{Section:Nested_decoder}. We will use ``candidate combinations'' and  ``helpful fragments'' to provide this high-level description. We say a combination of fragments is considered as a candidate combination if it satisfies all VT conditions in all layers with respect to its length. We let the empty set to be a candidate combination as well. Additionally, a fragment is called helpful if integrating that fragment with a candidate combination results in a new candidate combination.

The decoder begins its task by searching among all broken fragments to find the helpful fragment(s) and saves helpful fragments as candidate combinations. Then, it uses other fragments to find new helpful fragments and combines them with the candidate combination(s) to make a longer and longer candidate combinations. We continue this procedure until we attain $\hat{\textbf{x}}$ of length $n$ %(which may have missing pieces 
that meets all VT conditions. %\iscomment{how could it have missing pieces and be of length $n$?} 
We note that our nested VT decoder may find two or more candidate combinations of length $n$ that meet all the VT conditions. We will explain later in Section~\ref{subsect:VTdecoder_erasure_decoder} that we will use the overlap of these candidates plus an erasure code to recover the data.
%\iscomment{Ok}
Next, the decoder removes the parity bits to obtain $\hat{\textbf{d}}$. 

We allow the decoding algorithm to run for a limited timeframe, $\Delta$, an declare an error if the decoder obtains at least one output string during $\Delta$ and $\hat{\textbf{d}} \neq \textbf{d}$. In general, there will be some cases where our algorithm cannot find $\hat{\textbf{d}}$ within the given timeframe. In Section~\ref{Section:simulations}, we show that these cases represent a small fraction of the total cases and they decrease as we increase $\Delta$. %{\color{red} see my comment before conclusion.}

A natural question is whether it would be beneficial to consider other possibilities for $r_i^{(l)}$ such as using $r_i^{(l)}\neq 0$ or assigning different residues to each VT codeword within the nested structure. We will study this in Section~\ref{Section:simulations} and show that: (i) with $r_i^{(l)}\neq 0$, the decoding error increases; (ii) using different residues provides almost the same error rate, but slightly decreases the number cases where our algorithm cannot find $\hat{\textbf{d}}$ within $\Delta$.


\subsection{A new construction for a single VT Code}
\label{subsect:generate_VT_code}

In \cite{sloane2002single}, the author describes a VT encoder that generates codeword $\textbf{x}$ from data bits $\textbf{d}$ with linear complexity. More precisely, \cite{sloane2002single} constructs VT codeword $\textbf{x}$ as 
\begin{align}
\label{eq:construct_x}
\textbf{x}=[\textbf{d}~~\textbf{p}],
\end{align}
where $\textbf{d}$ is the data bits with length $n_d$, $\textbf{p}$ represents the parity bits with length $p$, and $p$ is equal to
\begin{align}
\label{eq:ParityLinear}
    p=\Bigg\lceil\sqrt{2n_d+\frac{9}{4}}+\frac{1}{2}\Bigg\rceil,
\end{align}
where $\ceil{.}$ is the ceiling function.

We note that~\cite{sloane2002single} does not provide a proof for this claim. % and in fact, it may not be a correct claim. {\color{red} please verify this sentence}

%{\color{blue} It is a correct statement. In Sloane's paper, the author mentioned neither how the number of parity bits is derived nor why the complexity of his approach is linear.}

In this paper, we propose a new encoding method for VT codes with a lower number of required parity bits compared to \eqref{eq:ParityLinear}. The following theorem quantifies the number of parity bits in our method. 

\begin{theorem}
\label{theorem_length_parity}
Given any data-bit sequence of length $n_d$, it is possible to construct a VT code as defined in (\ref{eq_VT_def}) of length $n$ with residue $0 \leq r \leq n$ where $n = n_d + p$ for $p=\Big\lceil\frac{1+\sqrt{1+8n_d}}{2}\Big\rceil$.
%\iscomment{for any residue $r$?}

\end{theorem}

\begin{proof}
The details are described in Appendix~\ref{appndx:thm_length_parity}.
\end{proof}

We provide a detailed description of how our VT encoder obtains parity bits $\mathbf{p}$ with linear complexity in Appendices~\ref{appndix:find_parity}  and \ref{appndix:complexity_parity}. %{\color{red} make sure the complexity is in fact linear.}

%{\color{blue} In appendix C, I revised the proof to show why our method's complexity is linear.}

\subsection{Encoding rate of the nested VT code}
\label{subsect:encoding_rate}
As we described above, in our proposed nested VT encoder, the lengths of input data bits $\textbf{d}$ and codeword $\textbf{x}$ are equal to $m^{(\ell-1)}d_{sec}$ and $n$, respectively. Hence, the encoding rate of our nested VT code is
\begin{align}
\label{eq_encoding_rate_def}
    R=\frac{m^{(\ell-1)}d_{sec}}{n}\overset{(a)}{=}\frac{m^{(\ell-1)}d_{sec}}{\Tilde{n}_{\ell}},
\end{align}
%\iscomment{I'm confused, doesn't the above imply that $n = \tilde{n}_\ell$?}

%\sncomment{Yes, it does. We use $\Tilde{n}_{\ell}$ to show the length of VT codeword in the last layer ($\ell^{\mathrm{th}}$ layer). Also, since the last layer of the nested VT code includes only one codeword, we have $n = \tilde{n}_\ell$.}
%\iscomment{Ok}
where $\Tilde{n}_{\ell}$ represents the length of the $\ell^{\mathrm{th}}$ layer, and $(a)$ holds true because the last layer of the nested VT code includes one codeword.
%\iscomment{I think the use of $\ell$ and $l$ in the description of the Nested VT encoder in the previous page is confusing. Is $\ell$ the total number of layers or a specific layer?}

%\sncomment{In our scheme, $\ell$ shows the total number of layers, and we use $l$ as an index that counts the different layers of nested VT code. Since $l=\ell$ in the last layer, we use $\ell$ to describe the corresponding parameters in $\ell^{\mathrm{th}}$ layer.}
%\iscomment{Ok}

Moreover, we know that each codeword in layer $l$, $1 \leq l \leq \ell$, contains $m$ different codewords of the $(l-1)^{\mathrm{th}}$ layer. As a result, we need the length of codewords in all layers to attain $\Tilde{n}_{\ell}$, which gives us a recursive formula. Below, we present the details.

The first layer of our encoder includes $m^{(\ell-1)}$ sections where the length of each section is equal to $d_{sec}$. Therefore, from Theorem~\ref{theorem_length_parity}, we have
\begin{align}
\label{tilda_n_1_main}
    \Tilde{n}_1=d_{sec}+\Bigg\lceil\frac{1+\sqrt{1+8d_{sec}}}{2}\Bigg\rceil,
\end{align}
where $\Tilde{n}_1$ is the length of each codeword in layer 1.

In the second layer, each codeword consists of $m$ different codewords of the first layer. Hence, we calculate $\Tilde{n}_2$ (the length of each codeword in layer 2), as
\begin{align}
\label{eq:n2_tilde_main}
   \Tilde{n}_2=m\Tilde{n}_1+\Bigg\lceil\frac{1+\sqrt{1+8m\Tilde{n}_1}}{2}\Bigg\rceil. 
\end{align}
Following the same rule, we have
\begin{align}
\label{eq:nl_tilde_main}
   \Tilde{n}_{\ell}=m\Tilde{n}_{\ell-1}+\Bigg\lceil\frac{1+\sqrt{1+8m\Tilde{n}_{\ell-1}}}{2}\Bigg\rceil. 
\end{align}

The following theorem
%We note that deriving a closed-form expression for $\Tilde{n}_{\ell}$ would not be possible due to the ceiling function. As a result, we use the following theorem to 
provides lower and upper bounds of the encoding rate of our nested VT code.


\begin{theorem}
\label{theorem:encoding_rate}
Given that $n_d=m^{(\ell-1)}d_{sec}$ is the length of data bits $\textbf{d}$ and for $d_{sec}\geq 36$, the encoding rate of the $\ell$-layered nested VT code is bounded by %{\color{red} (1) Instead of $R_1$ and $R_2$ use something like $\bar{R}$ and $\hat{R}$ or $R^-$ and $R^+$; (2) put $R_1$ and $R_2$ as equations, not in the text; (3) pick some parameters and plot the lower and upper bounds as well as the rate you actually get.}
\begin{align}
\label{eq:nested_rate_main_results}
R^-<R<R^+,
\end{align}
where 
\begin{align}
\label{eq:R_minus}
    R^-=\frac{m^{\ell-1}d_{sec}}{\Big(m^{(\frac{\ell-1}{2})}\sqrt{d_{sec}}+\frac{\sqrt{2.5}}{2}\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1}\Big)^2},
\end{align}
and the upper bound, $R^+$, is equal to
\begin{align}
\label{eq:R_plus}
    R^+=\frac{2m^{\ell-1}d_{sec}}{\Big(m^{(\frac{\ell-1}{2})}\sqrt{2d_{sec}}+\frac{m^{\frac{\ell}{2}}-1}{\sqrt{m}-1}\Big)^2}.
\end{align}
\end{theorem}
\begin{proof}
We defer the proof to Appendix~\ref{appndix_proof_encoding_rate}.
\end{proof}
In Fig.~\ref{Fig:encoding_rate_boundaries}, we describe how $R^-$, $R$, and $R^+$ behave when $\ell=3$ and $9\leq \log_2(n)<17$. Here, the encoding rate approaches $R^+$ as $n \to \infty$. %{\color{brown}
In general, we select $\ell$ based on $\alpha$, and then we let $d_{sec}\to\infty$ and $m\to\infty$ to capture $n\to\infty$. Specifically, in Fig.~\ref{Fig:encoding_rate_boundaries}, we set $\ell=3$ and increase $d_{sec}$ and $m$ to get the results.%} 
It is worth mentioning that $R$ describes the encoding rate and not the achievable rate. Of course, to have any hope of having vanishing error probability, we need $R < C$. Therefore, we always select $\ell$, $m$, and $d_{sec}$ such that $R < e^{-\alpha}$.%}

%\iscomment{when you let $n\to\infty$, how do $m$ and $\ell$ vary? are they fixed and $d_{sec}$ is growing?}

%\iscomment{Ok, but you may want to explain what happens to these parameters as $n \to \infty$.}

%\sncomment{I've added a statement above, highlighted in brown, to explain how $d_{sec}$ and $m$ vary as $n\to\infty$. Please find it.}

%\iscomment{Is $R$ growing to $1$ as $n\to \infty$? You may also want to mention how this rate relates to the capacity $e^{-\alpha}$, or say that it will be discussed later}

%\sncomment{Here, it seems that using \eqref{eq:nested_rate_main_results}, \eqref{eq:R_minus}, and \eqref{eq:R_plus} leads to $R \to 1$ as $n \to \infty$. However, as we discussed in Section~\ref{Section:intro}, the capacity of the chop-and-shuffle channel is equal to $C=e^{-\alpha}$. As a result, in this work, we always choose $m$, $\ell$, and $d_{sec}$ such that $R\leq C$.}\iscomment{Ok}
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.85\linewidth]{images/encoding-rate.png}
  \caption{\it The lower and upper bounds of the nested VT code encoding rate versus the actual encoding rate of nested VT code.\label{Fig:encoding_rate_boundaries}%\iscomment{is this figure mentioned in the text?} \sncomment{Yes, we describe it after \eqref{eq:R_plus}.}
  }
\end{figure}

==> sections/Section4_erasure_nested.tex <==
Ideally, we would like to recover $\textbf{x}$ perfectly; however, for various reasons we may not be able to obtain a unique sequence as the output of the decoder. %place all fragments in their correct place. A simple reason would be if the fragments are too short, then they can fit many different positions. This issue has been further investigated in~\cite{motahari2013information,TornPaperCoding,ravi2021coded}.
A simple reason would be some of the fragments could fit at different positions, and this results in multiple reassembled sequences as the outputs of the nested VT decoder that satisfy all VT conditions. While this may seem like an error at first glance, we take the overlap of all the outputs as the final reassembled sequence, and our simulations show this, if treated with care, will result in a correct reconstruction with high probability. Of course, taking the overlap results in some missing pieces, which can be viewed as erasures.
%}%, thus justifying the use of an erasure code.}
% in \cite{motahari2013information}, the authors show that it is impossible to recover all data bits if there is short fragment(s) with length less than $2\log_2(n)$, and this results in the loss of some data bits (i.e., missing fragments), as shown in Fig.~\ref{Fig:lost_databits}. 
%{\color{red} (1) Please be sure you understand what you cite! They do not show what you claim! (2) cite coded shotgun sequencing}

%{\color{blue}I used coded shotgun sequencing to write the previous claim. In that paper, the author says that \cite{motahari2013information} proves that it is impossible to recover all data bits if the read length is less than $2\log_2(n)$. But that claim holds for shotgun sequencing, where we read a fixed length of bits that may be overlapping.}

\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.7\linewidth]{images/non-recovered.png}
  \caption{\it If there are some fragments of very short length, the nested VT code fails to recover all data bits.\label{Fig:lost_databits}}
\end{figure}


As a result, to handle these erasures, we first apply an erasure code to the data bits %iscomment{bots?}
before feeding the sequence to the nested VT encoder. We note that since our nested VT code preserves the data structure (i.e., it places parity bits at the end of each codeword), we can apply the erasure code before our proposed encoder and data recovery will require an erasure decoder at the end. This way, the total rate of our scheme with erasure and nested VT codes is equal to 
\begin{align}
    R_t=(1-\epsilon)R,
\end{align}
where $(1-\epsilon)$ is the erasure code rate, and we will determine $\epsilon$ heuristically with simulations.

%where $R$ describes the rate of our nested VT code.

%{\color{brown}The reason we add an erasure code before using the nested VT code is as follows. First, our algorithm may fail to place all fragments in their corresponding correct place. This is especially the case when we face shorter and shorter fragments. Second, there could be multiple reassembled sequences as the outputs of the algorithm. While this may seem like an error at first glance, we take the overlap of all the outputs as the final reassembled sequence, and our simulations show this, if treated with care, will result in a correct reconstruction with high probability. Of course, taking the overlap results in more missing pieces, which can be viewed as erasures, thus justifying the use of an erasure code.}


As we mentioned in Section~\ref{Section:Main}, we need $R<C$ as a necessary condition to expect the error probability to decrease as $n$ increases in the chop-and-shuffle channel; thus, in our encoding scheme, we select $\ell$, $m$, and $d_{sec}$ such that $R < e^{-\alpha}$. Fig.~\ref{Fig:rate_our_vs_nested} compares the rate of the nested VT code plus erasure code with the baseline nested VT code where the value of $\epsilon$ is obtained heuristically.
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.9\linewidth]{images/our_versus_nested.eps}
  \caption{\it Comparison between the rate of nested VT code with and without the erasure code.\label{Fig:rate_our_vs_nested}}
\end{figure}

In Fig.~\ref{Fig:capacity_rates}, we compare the rate of our approach (i.e., erasure code + nested VT code) with the capacity and the lower-bound derived in~\cite{TornPaperCoding} using de Bruijn sequences. We observe that our approach provides a higher rate compared to the interleaved-pilot scheme of \cite{TornPaperCoding}.
%\iscomment{how is the achievable rate computed? Theorem 2 does not really talk about an achievable rate as a function of $\alpha$}
%\sncomment{We choose $\ell$, $m$, and $d_{sec}$ such that $R\leq e^{- \alpha}$.}
%\iscomment{This should be explained somewhere. It's confusing to the reader that Theorem 2 does not provide a rate as a function of $\alpha$, but it is plotted as a function of $\alpha$ in Figure 6.}
%\sncomment{We explained in the paragraph after Theorem 2 that ``$R$ describes the encoding rate and not the achievable rate. Of course, to have any hope of having vanishing error probability, we need $R < C$. Therefore, we always select $\ell$, $m$, and $d_{sec}$ such that $R < e^{-\alpha}$.''

%I also reminded the readers of this point at the beginning of this paragraph.}
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.9\linewidth]{images/Fig_rate_diff_alpha.eps}
  \caption{\it Comparison between the rate of nested VT code +erasure code, lower-bound of \cite{TornPaperCoding}, and the capacity. {\color{red} wait till the end and make sure the reference is cited correctly in the legend.} {\color{blue}Sure! I will update the reference number when everything is done.}\label{Fig:capacity_rates}}
\end{figure}


==> sections/Section5_description_NestedVT_encoder.tex <==
In this part, we present our proposed nested VT encoder with $\ell$ layers. %Furthermore, we show a lower bound on $d_{sec}$, which ensures to assign a unique residue to each codeword section in all layers. Below, we illustrate the details.
As we discussed in Section~\ref{Section:erasure_nested}, we need an erasure code before our nested VT code to compensate for the missing fragments at the end. Therefore, we build our encoder by concatenating an erasure encoder to the nested VT encoder as in Fig.~\ref{Fig:nested_encoder_scheme}.

\begin{figure}[!ht]
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=6, width=0.99\linewidth]{images/encoder_sch_r_0_without_r.png}
  \caption{\it Our encoding structure includes both erasure and nested VT codes.
  \label{Fig:nested_encoder_scheme}}
\end{figure}
\noindent \textbf{Initial processing}: Suppose $\textbf{w}$ is the binary input sequence. We apply an erasure code with the rate $0 \leq (1-\epsilon) \leq 1$ to $\textbf{w}$ to obtain $\textbf{d}$ as the input sequence to our nested VT encoder. For simplicity, we will refer to $\textbf{d}$ as data bits. As mentioned before, the rate for the erasure code will be determined heuristically;

%{\color{red} ``to simulate missing fragments'' does not make any sense. See how I wrote the paragraph above and revise wherever applies.}

%{\color{blue} Thank you for your comment. This is the only place where I use ``to simulate missing fragments''.}


\noindent $\textbf{Breaking the input data bits d into~} \mathbf{m^{\ell-1}~}\textbf{sections:}$ The nested VT encoder breaks $\textbf{d}$ with length $n_d=m^{(\ell-1)}d_{sec}$ into $m^{(\ell-1)}$ data sections where the length of each data bits section is equal to $d_{sec}$; %We use $\textbf{d}_i^{(l)}$ to denote the $i^{\text{th}}$ section of data bits in layer $l, 1 \leq l \leq \ell$;

\noindent $\textbf{Encode each data section:}$ In this step, we apply VT code on each data section $\textbf{d}^{(l)}_i, 1 \leq l \leq \ell, 1 \leq i \leq m^{\ell-l}$ to obtain VT codeword $\textbf{x}^{(l)}_i$. To do this, in the $i^{\mathrm{th}}$ section of data bits in layer $l$, we use residue $r_i^{(l)}=0, 1 \leq i \leq m^{(\ell-l)}$ to encode data section $\textbf{d}^{(l)}_i$. 
% Based on Lemma~\ref{lemma_d_sec}, we choose $d_{sec}$ such that $d_{sec}+\ceil{\frac{1+\sqrt{1+8d_{sec}}}{2}}\geq m^{(\ell-1)}-1$ in order to have unique residue values to encode each data section in the first layer. 

\noindent $\textbf{Combining the codewords:}$ In layer $l, 2 \leq l \leq \ell$, we merge every $m$ VT codewords of layer $(l-1)$ to create a new data section. Specifically, we set 
\begin{align}
    \textbf{d}_i^{(l)}=[\textbf{x}_{i}^{(l-1)}, \textbf{x}_{i+1}^{(l-1)}, \ldots, \textbf{x}_{i+m-1}^{(l-1)}], \quad 1 \leq i \leq m^{\ell-l}.
\end{align}
We use these new sections as the input of the VT encoder in layer $l$. This way, the number of data bits sections is reduced by a factor of $m$ in each layer. Then, we use the same approach to encode the data-bit sections in the new layer. The VT codeword of layer $\ell$ will be the output of the nested VT encoder. 
   
Moreover, we present a pseudo code in Algorithm~\ref{algo:algo_encode} to describe how our proposed encoder runs the encoding procedure.
%%-----------------%%
\begin{algorithm}
  \caption{Encoding Algorithm}
    \label{algo:algo_encode}
  \begin{algorithmic}[1]
  \State Attain $\textbf{d}$ applying an erasure code with rate $1-\epsilon$ to $\textbf{w}$;\
  \State Break $\textbf{d}$ into $m^{(\ell-1)}$ sections as $\textbf{d}^{(1)}_i$;\
  \For{$l\in [1,\ell]$}
    \For{$i\in [1,m^{(\ell-l)}]$}
        \State {Encode $\textbf{d}^{(l)}_i$ to a VT codeword as $\textbf{x}^{(l)}_i$ based} $~~~~~~~~~$ \hspace{1.1pt}{\color{white}123456}on residue $r_i^{(l)}=0$;\
    \EndFor
    \If{$l\neq \ell$}
    \State {Merge every $m$ codewords in layer $l$ to create} $~~~~~~~~~$ \hspace{-1.1pt} {\color{white}123456}a new data-bit section in layer $l+1$;\
    \EndIf
  \EndFor
  \State Consider $\textbf{x}=\textbf{x}_1^{(\ell)}$ as the nested VT codeword.
\end{algorithmic}
\end{algorithm}
%%-----------------%%
First, we use an erasure encoder and convert initial data bits $\textbf{w}$ into $\textbf{d}$. In the second line of Algorithm~\ref{algo:algo_encode}, we break the input data bits $\textbf{d}$ into $m^{(\ell-1)}$ sections, $\textbf{d}^{(1)}_i$. Next, in each encoding layer, we do the following tasks: (1) We encode each $\textbf{d}^{(l)}_i$ as VT codeword $\textbf{x}^{(l)}_i$ based on a fixed residue ($r_i^{(l)}=0$); (2) If $l \neq \ell$, we combine every $m$ VT codewords together to create a new data-bit section for the next layer. Finally, we define the output of the last layer as the nested VT codeword $\textbf{x}$.


%{\color{brown}
Notice that although we design the nested VT code by deploying $r_i^{(l)}=0$ for all codewords, one possible question is what occurs if we use other methods such as $r_i^{(l)}\neq 0$ or different unique residues as $r_i^{(l)}=i-1$ for each codeword in each layer? To answer this, we will compare the decoding error of using $r_i^{(l)}=0$, $r_i^{(l)} \neq 0$, and different residues in Section~\ref{Section:simulations}. We will describe that using different residues slightly reduces the number of cases where the decoder fails to find a solution during limited time $\Delta$, and using the same {\it non-zero} residue would increase the error rate. %{\color{red} I changed the last phrase, make sure it is correct and remove this comment.}

\subsection{An example of the nested VT encoder}
We provide an example in Fig.~\ref{Fig:ex_nested_encoder} with $\ell=2$ layers and $m=2$ to illustrate our nested VT encoder. Here, we focus on the nested VT encoder and remove the erasure encoder to simplify the descriptions. We consider $\textbf{d}=[1~1~0~1~0~1~1~1~0~1~0~1~1~1]$ as the input data bits with $n_d=14$ and $d_{sec}=7$. To encode the data bits, we break $\textbf{d}$ into $m^{\ell-1}=2$ sections as $\textbf{d}_1^{(1)}=[1~0~1~1~0~0~1]$ and $\textbf{d}_2^{(1)}=[1~0~1~0~1~0~0]$. Then, we apply a VT code with $r_1^{(1)}=0$ to $\textbf{d}_1^{(1)}$ to obtain $\textbf{x}_1^{(1)}=[1~0~1~1~0~0~1~0~0~0~1~0]$. Similarly, we get $\textbf{x}_2^{(1)}=[1~0~1~0~1~0~0~1~1~0~0~00]$ using $r_2^{(1)}=0$. In the second layer, we merge $\textbf{x}_1^{(1)}$ and $\textbf{x}_2^{(1)}$ to construct $\textbf{d}_1^{(2)}=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~1~0~1~0~0~1~1~0~0~0]$ as the only data-bit section in that layer. Finally, we apply a  VT code with residue $r_1^{(2)}=0$ to attain $\textbf{x}=\textbf{x}_1^{(2)}=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~1~0~1~0~0~1~1~0~0~0~1~0~0~1~0~0~0~0]$ as the nested VT codeword. %\iscomment{nice example}
%\sncomment{Thank you, Dr. Ilan!}
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/encoder_example_r_0.png}
  \caption{\it An example of nested VT encoder when $\ell=2$, $m=2$, and $d_{sec}=7$.\label{Fig:ex_nested_encoder}}
\end{figure}

%\iscomment{In general, it was a bit unclear to me why unique residues are needed. It was also unclear why checking the VT conditions is a good way to find the correct ordering of the pieces. In other words, why do we expect that an incorrect ordering will not satisfy the VT conditions? That seems expected, but it would be good to discuss it.
%Also, why would we expect to recover the correct ordering of the fragments with some missing fragments? wouldn't the missing fragments cause the VT conditions to be violated?}

%\sncomment{Thank you, Dr. Ilan for your comment! I ran the simulations with a fixed residue ($r_i^{(l)}=0$) for all VT codewords in all layers. The results show that the complexity of using unique residues is slightly better than using a fixed residue, and the decoding error of both methods is almost the same. Thus, I've updated the results based on $r_i^{(l)}=0$ throughout the paper.

%Also, I've added a paragraph in Section~\ref{Section:erasure_nested} describing our nested VT decoder may find two or
%more candidate combinations of length $n$ that meet all VT
%conditions. In this case, we take the
%overlap of all the outputs as the final reassembled sequence. We note that
%taking the overlap results in some missing pieces, which can
%be interpreted as erasures. As a result, we need an erasure code in our scheme to tackle these missing pieces.}

%\iscomment{Ok}

% \subsection{Unique residue}
% \label{subsect:unique_res}
% We use the following lemma to determine a lower bound on $d_{sec}$ in order to ensure a unique residue can be assigned to each codeword.

% \begin{lemma}
% \label{lemma_d_sec}
% To ensure $r^{(l)}_i=i-1$ is a unique residue used for the $i^{\mathrm{th}}$ codeword in the $l^{\mathrm{th}}$ layer of nested VT code, for $\ell\geq 1 $ and $m\geq 2$, we need 
% \begin{align}
% d_{sec}\geq m^{(\ell-1)}-\sqrt{2m^{(\ell-1)}-1}.
% \end{align}
% \end{lemma}

% \begin{proof}
% Since the $l^{\mathrm{th}}$ layer of our nested VT code has $m^{\ell-l}$ sections where $1 \leq l \leq \ell$, the first layer of our code requires the highest number of unique residues. This means that if we have a unique residue for each section of the first layer, all other layers will have the sufficient number of unique residues. As a result, in this proof, we focus on the residues of the first layer to obtain a lower bound on $d_{sec}$.

% According to Theorem~\ref{theorem_length_parity}, the length of each VT codeword in the first layer is equal to
% \begin{align}
%     \Tilde{n}_1=d_{sec}+\Bigg\lceil\frac{1+\sqrt{1+8d_{sec}}}{2}\Bigg\rceil,
% \end{align}
% and based on \eqref{eq_VT_def}, we have $0\leq r_i^{(1)} \leq d_{sec}+\Big\lceil\frac{1+\sqrt{1+8d_{sec}}}{2}\Big\rceil$.

% Moreover, we have $m^{(\ell-1)}$ different VT codewords in the first layer where $r_i^{(1)}=i-1$; therefore, $0\leq r_i^{(1)} \leq m^{(\ell-1)}-1$. 

% As a result, to dedicate a unique residue to each VT codeword in the first layer, we should select $d_{sec}$ such that 
% \begin{align}
% \label{eq:dsec_cond}
%     d_{sec}+\Bigg\lceil\frac{1+\sqrt{1+8d_{sec}}}{2}\Bigg\rceil\geq m^{(\ell-1)}-1.
% \end{align}

% %{\color{red} This is not correct. Below you show RHS of (20) is greater than something, why should that something be greater than the LHS of (20)?! You should *upper bound* the LHS of (20) by removing the ceiling function and adding a ``1''. Then, that upper-bound is also greater than the RHS of (20).}

% In addition, we have
% \begin{align}
% \label{eq:dsec_lower_bound}
%     d_{sec}+\Bigg\lceil\frac{1+\sqrt{1+8d_{sec}}}{2}\Bigg\rceil&\geq d_{sec}+\frac{1+\sqrt{1+8d_{sec}}}{2} \\ \nonumber
%     &>d_{sec}+\sqrt{2d_{sec}}.
% \end{align}
% Thus, any $d_{sec}$ that satisfies
% \begin{align}
% \label{eq:approx_d_sec}
%     d_{sec}+\sqrt{2d_{sec}}\geq m^{(\ell-1)}-1,
% \end{align}
% will also satisfy \eqref{eq:dsec_cond}. Consequently, we use $\Tilde{d}_{sec}=\sqrt{2d_{sec}}$ and rewrite \eqref{eq:approx_d_sec} as
% \begin{align}
% \label{eq:dsec_cond2}
%     \frac{\Tilde{d}_{sec}^2}{2}+\Tilde{d}_{sec}\geq m^{(\ell-1)}-1.
% \end{align}
% We can show that the inequality condition in \eqref{eq:dsec_cond2} holds either $\Tilde{d}_{sec}\leq -\sqrt{2m^{(\ell-1)}-1}-1$ or $\Tilde{d}_{sec}\geq \sqrt{2m^{(\ell-1)}-1}-1$, where the former is not correct since $\Tilde{d}_{sec}$ is a positive number. Therefore, applying $\Tilde{d}_{sec}= \sqrt{2d_{sec}}$ to \eqref{eq:dsec_cond2} leads to
% \begin{align}
% \label{eq:dsec_cond3}
%     d_{sec}\geq m^{(\ell-1)}-\sqrt{2m^{(\ell-1)}-1}.
% \end{align}
% As a result, \eqref{eq:dsec_cond3} provides a lower bound on $d_{sec}$ that meets the condition in \eqref{eq:dsec_cond}, and this completes the proof.
% \end{proof}

==> sections/Section6_description_NestedVT_decoder.tex <==
% As we discussed in Section~\ref{Section:erasure_nested}, our proposed encoder/decoder use an erasure code and the nested VT code together to encode/retrieve data bits. Therefore, 
%In this section, we divide the explanations of our decoder into two parts:
%{\color{red} you say you break it into two parts, but there are three subsections and they do not seem to be divisions of the topic at all. You may wanna say we first look at an idealized decoder where ... and then explain how those issues can be handled... The subsections hsould follow that description.}

To explain how our proposed decoder works, we first look at an idealized decoder where the decoding algorithm finds only one permutation of the fragments as the recovered codeword. We also provide an example to demonstrate the details. Then, we discuss how we incorporate erasure codes in non-ideal scenarios. Further details are provided below.

\subsection{Ideal nested VT decoder}
In this part, we focus on an ideal nested VT decoder as shown in Fig.~\ref{Fig:nested_decoder}, which reconstructs only one permutation of the fragments as the recovered codeword. We assume the chop-and-shuffle channel breaks codeword $\textbf{x}$ into $M$ fragments with random lengths and then shuffles these fragments. To track the fragments during the process, we allocate $M$ labels as $\mathbf{y}_j, j=1,2,\ldots, M$ to the fragments. Before describing in detail, we define some parameters to be used in decoding.

\textbf{Matrix $\mathbf{N}$:} This matrix represents the position of the last bit in all VT codewords in all layers. The size of this matrix is $\ell \times m^{(\ell-1)}$ where $l^{\mathrm{th}}$ row has $m^{(\ell-l)}$ non-zero elements, corresponding to $m^{(\ell-l)}$ codewords in layer $l$, and $N_{l,i}, 1\leq l \leq \ell, 1\leq i \leq m^{(\ell-l)}$ shows the position of the last bit in $\textbf{x}_i^{(l)}$. For example, suppose $d_{sec}=24$, $m=2$, and $\ell=4$, then matrix $\mathbf{N}$ is equal to
\begin{align}
\label{eq:matrix_N}
    \mathbf{N}=
\begin{bmatrix}
32 &  64 & 108 & 140 & 202 & 234 & 278 & 310 \\
76 &  152 & 246 & 322 & 0 & 0 & 0 & 0 \\170 &  340 & 0 & 0 & 0 & 0 & 0 & 0 \\
367 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\end{bmatrix},
\end{align}

%{\color{brown}
where $32$ is the length of $\textbf{x}^{(1)}_1$ that is obtained using Theorem~\ref{theorem_length_parity} and $d_{sec}=24$. Furthermore, we know that $\textbf{x}^{(1)}_2$ is the next codeword in $\textbf{x}$ with length $32$; therefore, the position of the last bit in $\textbf{x}^{(1)}_2$ is equal to $32+32=64$. Then, since $m=2$, every two codewords in layer 1 are merged together to create a new data bits section in layer 2. Thus, $\textbf{d}^{(2)}_1=[\textbf{x}^{(1)}_1~~ \textbf{x}^{(1)}_2]$ with length $64$, and using $\textbf{d}^{(2)}_1$ and Theorem~\ref{theorem_length_parity} leads to have $\textbf{x}^{(2)}_1$ with length $76$. We can get other numbers in matrix $\mathbf{N}$ by following the same rule.


%{\color{brown}As we described above, to derive each element of matrix $\mathbf{N}$, we need the length of the corresponding data bits section and Theorem~\ref{theorem_length_parity}. As a result, we can find the position of the first bit of any VT codeword subtracting its length from the position of its last bit in matrix $\mathbf{N}$.}
%}
%\iscomment{can you explain how some of these numbers are generated? for example, how is 32 and 64 obtained from the parameters above?}
%\iscomment{Ok}


\textbf{Candidate combination:} Suppose $\boldsymbol\Gamma$ is a sequence that can be generated from the elements of $S(\mathbf{x})$ and $|\boldsymbol\Gamma|$ is the size of $\boldsymbol\Gamma$ where $0\leq |\boldsymbol\Gamma|\leq M$. Here, we use $\gamma$ to denote the length of $\boldsymbol\Gamma$. More precisely, we have
\begin{align}
    \gamma=\sum_{j^{\prime}=1}^{|\boldsymbol\Gamma|} L_{j^{\prime}}, \quad \mathbf{y}_{j^{\prime}}\in \boldsymbol\Gamma,
\end{align}
where $L_{j^{\prime}}$ is the length of $\mathbf{y}_{j^{\prime}}$. Notice that $\gamma=0$ if $|\boldsymbol\Gamma|=0$. Then, we check the VT condition of every codeword $\textbf{x}^{(l)}_i, 1\leq l \leq \ell, 1\leq i \leq m^{(\ell-l)}$ corresponding to element $N_{l,i}$ in matrix $\mathbf{N}$ if $N_{l,i}\leq \gamma$. Finally, we call $\boldsymbol\Gamma$ a candidate combination if it satisfies VT conditions for all the above codewords. 

% {\color{red} I am a bit confused. We do not know the order obviously. So, what do you mean by ``a codeword corresponding to element $N_{l,i}$ in matrix $\mathbf{N}$''? This way you are back again to the same mistake. We discussed and there should be at least one subset of the correct size to satisfy the VT conditions in a CC. Am I misreading this?}

We demonstrate an example to make the definition of a candidate combination clear. Consider $d_{sec}=24$, $m=2$, $\ell=4$, and $\boldsymbol\Gamma$ is a sequence of some fragments in $S(\mathbf{x})$ with length $\gamma=153$. By using matrix $\mathbf{N}$ in \eqref{eq:matrix_N}, we find that $N_{1,1}=32, N_{1,2}=64, N_{1,3}=108, N_{1,4}=140, N_{2,1}=76$, and $N_{2,2}=152$ are smaller than $\gamma=153$. Therefore, if $\boldsymbol\Gamma$ meets VT conditions of $\textbf{x}^{(1)}_1,\textbf{x}^{(1)}_2, \textbf{x}^{(1)}_3, \textbf{x}^{(1)}_4, \textbf{x}^{(2)}_1$, and $\textbf{x}^{(2)}_2$, it will be a candidate combination.


\begin{comment}
{\color{brown}Suppose $\bar\Pi(S(\mathbf{x})) \subseteq S(\mathbf{x})$ and $\Pi(S(\mathbf{x}))$ is an ordering on $\bar\Pi(S(\mathbf{x}))$ with length $|\Pi(S(\mathbf{x}))| \in \mathbb{Z}^+$ where $0<|\Pi(S(\mathbf{x}))|\leq n$.} Then, by looking at matrix $\mathbf{N}$, we obtain the closest numbers to $|\Pi(S(\mathbf{x}))|$ in each row of $\mathbf{N}$ as $\hat N_{1,i_1}, \hat N_{2,i_2}, \ldots, \hat N_{l,i_l}, \ldots, \hat N_{\ell,i_{\ell}}$ where $\hat N_{l,i_l}\leq |\Pi(S(\mathbf{x}))|, 1 \leq l \leq \ell, 1\leq i_l\leq m^{(\ell-l)}$ denotes the closest number to $|\Pi(S(\mathbf{x}))|$ in $l^{\mathrm{th}}$ row of $\mathbf{N}$, which is available in ${i_l}^{\mathrm{th}}$ column of $\mathbf{N}$. Notice that: (1) $\hat{N}_{l,i_l}$ indicates the position of the last bit of VT codeword $\mathbf{x}^{(l)}_{i_l}$, which may be constructed by $\Pi(S(\mathbf{x}))$; (2) if there is no $\hat N_{l,i_{l}}\neq 0$, $\Pi(S(\mathbf{x}))$ does not include a VT codeword in layers $l, l+1, \ldots, \ell$; thus, we do not need to check the VT conditions in layers $l, l+1, \ldots, \ell$. Here, we call $\Pi(S(\mathbf{x}))$ a candidate combination if it satisfies all VT conditions corresponding to all VT codewords in all layers created by $\Pi(S(\mathbf{x}))$. 
\iscomment{I didn't understand the definition of Candidate combination. Not clear how $\mathbf{N}$ is used to find $\hat N_{l,i}$ or what $\gamma$ represents (are we just looking at fragments with a specific length $\gamma$?)}

\sncomment{I've revised the definition of a candidate combination above. Please check the details.}

\iscomment{Things are still unclear to me. Can you formally define what $\Pi(S(x))$ is? The word ``combination'' is not very specific. I'm also confused by the role of $\gamma$. Why do you define $\Pi(S(x))$ for a specific fragmenet length $\gamma$? Shouldn't $\Pi$ just be an ordering on the entire set of fragments $S(x)$? What if all fragments have unique lengths?}
\sncomment{Thank you, Dr. Ilan for this comment! I updated the above paragraph using the following definition on $\Pi(S(x))$.

``Suppose $\bar\Pi(S(\mathbf{x})) \subseteq S(\mathbf{x})$ and $\Pi(S(\mathbf{x}))$ is an ordering on $\bar\Pi(S(\mathbf{x}))$ with length $|\Pi(S(\mathbf{x}))| \in \mathbb{Z}^+$ where $0<|\Pi(S(\mathbf{x}))|\leq n$.''

I also used $|\Pi(S(\mathbf{x}))|$ instead of $\gamma$ in the revised paragraph to show the length of $\Pi(S(\mathbf{x}))$. Here, $|\Pi(S(\mathbf{x}))|$ doesn't mean that we choose $\Pi(S(\mathbf{x}))$ such that its length is equal to any specific value. On the contrary, we use $\Pi(S(\mathbf{x}))$ just to represent the length of $\Pi(S(\mathbf{x}))$ where $\Pi(S(\mathbf{x}))$ could be any permutation of $\bar\Pi(S(x))$ with its corresponding length.}

\iscomment{I'm still confused. Probably not a good idea to have $\bar{\Pi}(S(x))$ being a different kind of object than $\Pi(S(x))$.
I'm also confused by the meaning of $|\Pi(S(x))|$. This makes it look like $\Pi(S(x))$ is a set, and $|\Pi(S(x))|$ is the cardinality of that set.
Is that correct? 
Or is $|\Pi(S(x))|$ the length of the fragments in $\Pi(S(x))$? That's not good notation.
Also, why is it that you focus on a set of fragments with a given fragment length? I don't understand that.
}\end{comment}


\begin{remark}
We note that any sequence that is generated from the elements of $S(\mathbf{x})$ with a length less than $N_{1,1}$ (position of the last bit in $\textbf{x}_1^{(1)}$) is also a candidate combination because it includes no codeword and needs to wait for other fragments in future steps.
\end{remark}
\begin{remark}
For consistency, we consider $\phi$ (empty sequence) as a candidate combination in the first round of decoding. 
%There is no known candidate combination in the first round of decoding; therefore, we consider $\phi$ (empty {\color{brown}sequence}) as a candidate combination in the first round of decoding.
\end{remark} 
\textbf{Helpful fragment} We say $\mathbf{y}_j$ with length $L_j$ is a helpful fragment if the combination of $\mathbf{y}_j$ and any candidate combination creates a new candidate combination. 

\textbf{Limited memory:} As $\alpha$ increases, the number of fragments increases and the length of fragments decreases. Thus, our decoder requires to check a fast-growing number of possible cases, resulting in higher computational complexity. To tackle this issue, we define a limited memory with parameter $\tau \in \mathbb{Z}^+$. After every $\tau$ iterations, our algorithm keeps the candidate combinations with the highest number of satisfied VT conditions. If the algorithm cannot resume with any of the kept candidate combinations in the subsequent iterations, it increases $\tau$ by one and repeats the process.  Our simulation results show that this method reduces the complexity of our approach significantly compared to a brute-force search, see Section~\ref{Section:simulations}. 

As a high-level overview, our decoder runs multiple rounds of a searching algorithm between all fragments to find $\mathbf{\hat{\textbf{x}}}$, which satisfies all VT conditions. In the first round, it searches through all fragments to get helpful fragment(s) and consequently candidate combinations. Then, the decoder seeks to detect new helpful fragment(s) to integrate with candidate combinations to create new longer candidate combinations. Finally, the decoder finds $\mathbf{\hat{\textbf{x}}}$ if it is a candidate combination with length $n$. 
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/decod_p2.png}
  \caption{\it Ideal nested VT decoder\label{Fig:nested_decoder}}
\end{figure}

When our decoder obtains $\mathbf{\hat{\textbf{x}}}$, the rest of the decoding procedure will be simple. In particular, the decoder removes the parity bits from $\mathbf{\hat{\textbf{x}}}$ to get $\mathbf{\hat{\textbf{d}}}$. In Algorithm~\ref{algo:decoder}, we demonstrate how our ideal nested VT decoder performs the decoding procedure.

% The idea of our decoder is to combine as much as possible fragments in correct order to reduce the number of possible permutations. First, we run a pre-processing procedure to find any combination of the fragments which meet VT conditions in lower layers. Then, we consider these combinations as new fragments. Second, we sort the remained fragments in descending order and apply our decoder schemes to find exact position(s) of sufficiently large fragments (which will be explained in algorithm 3). Finally, we check all permutations of undetermined fragments to find a guess of encoded codeword as $\mathbf{\hat{\textbf{x}}}$. We divide our decoding scheme into three phases as below:

% \noindent $\textbf{Phase I:}$ We perform the pre-processing procedure as the first stage in our decoder scheme to find any combination of fragments which reduces the number of fragments (see Algorithm~\ref{algo:decoder}).

%%-----------------%%
\begin{algorithm}
  \caption{Decoding Algorithm}
  \label{algo:decoder}
  \begin{algorithmic}[1]
  \State $K=1$;\
  \State $\tau=1$;\
  \State $\boldsymbol\Gamma_1=\phi$;\
  \State $\beta_1=S(\mathbf{x})$;\
  \State $\tau^{\prime}=0$;\
  \For{$k \in [1,K]$}{
  %\State $\beta=$ Fragments $\in \{S(\mathbf{x})\setminus CC_k\}$;\ 
  \State $Rep_k=0$;\
  \For{$\mathbf{y}_j \in \beta_k$}{
  \State $\boldsymbol\Gamma^{\prime}=[\boldsymbol\Gamma_k ~~\mathbf{y}_j]$;\
  \If{$\boldsymbol\Gamma^{\prime}$ is a candidate combination}
  \State $Rep_k \leftarrow Rep_k+1$;
  \State $\boldsymbol\Gamma_{K+Rep_k}=\boldsymbol\Gamma^{\prime}$;\
  \State \hspace{-10pt} $\beta_{K+Rep_k}=$ Fragments $\in \{S(\mathbf{x})\setminus \boldsymbol\Gamma_{K+Rep_k}\}$;\ 
  \If{Length $\boldsymbol\Gamma_{K+Rep_k}=n$}
  \State $\hat{\textbf{{x}}}=\boldsymbol\Gamma_{K+Rep_k}$;\
  \State Go to line 30;\
  \EndIf
  \EndIf
  }
  \EndFor
  }
  \EndFor
  \For{$k \in [1,K]$}
  \State Remove $\boldsymbol\Gamma_k$;\
  \EndFor
  \State $\tau^{\prime}\leftarrow\tau^{\prime}+1$;\
  \If{$\tau^{\prime}\geq \tau$}
  \State Save the $\boldsymbol\Gamma_k$(s) with the highest number of\\ {\color{white}12~}\hspace{1pt}satisfied VT conditions;\
  \State $\tau^{\prime}=0$;\
  \EndIf
  \State Update $K$ as the number of candidate combinations;\
  \If{$K=0$}
  \State $\tau \leftarrow \tau+1$;\
  \State Go to line 1;\
  \Else
  \State Go to line 6;\
  \EndIf
  \State $l=\ell$
  \While{$l> 1$}
  \For{$i\in [1,m^{(\ell-l)}]$}
  \State Remove parity bits from $\mathbf{\hat{\textbf{x}}}^{(l)}_i$ to get $\mathbf{\hat{\textbf{d}}}^{(l)}_i$;\ 
%   where $\mathbf{\hat{\textbf{d}}}^{(l)}_i=[\mathbf{\hat{\textbf{x}}}^{(l-1)}_i, \mathbf{\hat{\textbf{x}}}^{(l-1)}_{i+1}, \ldots, \mathbf{\hat{\textbf{x}}}^{(l-1)}_{i+m-1}]$;\ 
  \State Break $\mathbf{\hat{\textbf{d}}}^{(l)}_{i}$ into $m$ parts $\mathbf{\hat{\textbf{x}}}^{(l-1)}_i$, $\mathbf{\hat{\textbf{x}}}^{(l-1)}_{i+1}$,$\ldots$, $\mathbf{\hat{\textbf{x}}}^{(l-1)}_{i+m-1}$;\
  \EndFor
  \State $l\leftarrow l-1$;\
  \EndWhile
  \State Decode $\hat{\textbf{d}}^{(1)}_i$ from $\hat{\textbf{x}}^{(1)}_i$ for all $1 \leq i \leq m^{(\ell-1)}$;\
  \State Combine $m^{\ell-1}$ data sections, as $\mathbf{\hat{\textbf{d}}}$.
\end{algorithmic}
\end{algorithm}
%%-----------------%%
Algorithm~\ref{algo:decoder} consists of three main parts: In lines 6 to 18, it searches among fragments to attain helpful fragments and candidate combinations. Then, in lines 19 to 29, the algorithm stores candidate combinations with the highest number of satisfied VT conditions and checks the limited memory of the searching algorithm. Finally, it deletes the parity bits from the estimated VT code to decode the data bits. Below, we explain the details.

%%%ALIREZA%%%

We initialize the algorithm using $K=1$, $\tau=1$, $\boldsymbol\Gamma_1=\phi$, $\beta_1=S(\mathbf{x})$, and $\tau^{\prime}=0$ where $K$ is the number of candidate combinations, $\tau$ represents the limited memory, $\boldsymbol\Gamma_k, 1 \leq k \leq K$ illustrates the $k^{\mathrm{th}}$ candidate combination, $\beta_k, 1 \leq k \leq K$ shows the fragments $\in \{S(\mathbf{x})\setminus \boldsymbol\Gamma_k\}$, and $\tau^{\prime}$ is an index that follows the limited memory. Next, for each $\boldsymbol\Gamma_k$, we define $Rep_k$, initialized to zero, to denote the number of new candidate combinations constructed by $\boldsymbol\Gamma_k$. Then, in line 8, we search between all $\mathbf{y}_j \in \beta_k$ to find the helpful fragments and set $\boldsymbol\Gamma^{\prime}=[\boldsymbol\Gamma_k~~\mathbf{y}_j ]$. If $\boldsymbol\Gamma^{\prime}$ is a candidate combination we increase $Rep_k$ by one, add $\boldsymbol\Gamma^{\prime}$ as a new candidate combination, and consider $\beta_{K+Rep_k}=$ fragments $\in \{S(\mathbf{x})\setminus \boldsymbol\Gamma_{K+Rep_k}\}$. Then, we check the length of $\boldsymbol\Gamma_{K+Rep_k}$. If its length is equal to $n$ we say $\hat{\mathbf{x}}=\boldsymbol\Gamma_{K+Rep_k}$ and go to line 30. After checking all candidate combinations, we remove the first $K$ candidate combinations because these $K$ candidate combinations create new candidate combinations with more elements in lines 6 to 16. Then, in line 19, we increase index $\tau^{\prime}$ by one and check whether we have used the whole memory or not. If so, we keep only those $\boldsymbol\Gamma_k(s)$, which provide the highest number of satisfied VT conditions and put $\tau^{\prime}=0$. Next, we update the number of candidate combinations. In line 25, if $K=0$, we realize that no candidate combination met the VT conditions using $\tau$ iterations. Hence, we set $\tau=\tau+1$ and restart the decoding procedure. Otherwise, we go to line 6 and continue with the remained candidate combinations. 

It is worth mentioning that the searching procedure between fragments is done when the decoder obtains a $\boldsymbol\Gamma_{K+Rep_k}$ with length $n$. Then, we call $\boldsymbol\Gamma_{K+Rep_k}$ as $\hat{\mathbf{x}}$ and removes its parity bits during lines 30 to 37. Specifically, we set $l=\ell$ and while $l>1$ do the following: For $i^{\mathrm{th}}$ codeword in $l^{\mathrm{th}}$ layer, where $1\leq i \leq m^{(\ell-l)}$, we remove the parity bits from the end of $\hat{\textbf{x}}^{(l)}_i$ to decode $\hat{\textbf{d}}^{(l)}_i$. In the next line, we break $\hat{\textbf{d}}^{(l)}_i$ into $m$ sections and consider each section as a codeword of layer $l-1$. Next, we decrease $l$ by one and repeat lines 32 to 34. Then, we recover $m^{(\ell-1)}$ data sections of layer 1 by just removing the parity bits from corresponding codewords in layer 1. Finally, we merge these $m^{(\ell-1)}$ data sections and obtain $\hat{\textbf{d}}$.

\subsection{An example of a nested VT decoder}
We use the same codeword of Fig.~\ref{Fig:ex_nested_encoder} as the VT nested codeword $\textbf{x}$. We consider an example where $\textbf{x}$ goes through the chop-and-shuffle channel and breaks into $M=3$ different pieces as Fig.~\ref{Fig:ex_nested_decoder}. Then, the decoder searches through all permutations to find a string that satisfies all VT conditions. As we can see in Fig.~\ref{Fig:ex_nested_decoder}, the decoder finds $\hat{\textbf{x}}=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~1~0~1~0~0~1~1~0~0~0~1~0~0~1~0~0~0~0]$ as the estimated version of the nested VT codeword. We know that $\hat{\textbf{x}}=\hat{\textbf{x}}_1^{(2)}$. So, the decoder removes parity bits and obtains $\hat{\textbf{d}}_1^{(2)}=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~1~0~1~0~0~1~1~0~0~0]$. Furthermore, we know that $\hat{\textbf{d}}_1^{(2)}$ includes two VT codewords of the first layer. Therefore, we divide $\hat{\textbf{d}}_1^{(2)}$ into two codewords $\hat{\textbf{x}}_1^{(1)}=[1~0~1~1~0~0~1~0~0~0~1~0]$ and $\hat{\textbf{x}}_2^{(1)}=[1~0~1~0~1~0~0~1~1~0~0~0]$. In this stage, we remove parity bits of $\hat{\textbf{x}}_1^{(1)}$ and $\hat{\textbf{x}}_2^{(1)}$ to attain $\hat{\textbf{d}}_1^{(1)}=[1~0~1~1~0~0~1]$ and $\hat{\textbf{d}}_2^{(1)}=[1~0~1~0~1~0~0]$. We know that estimated data bits $\hat{\textbf{d}}$ is created by combining $\hat{\textbf{d}}_1^{(1)}$ and $\hat{\textbf{d}}_2^{(1)}$. As a result, we have $\hat{\textbf{d}}=[1~0~1~1~0~0~1~1~0~1~0~1~0~0]$, which is the correct reconstruction.

\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/decoder_example_r_0.png}
  \caption{\it An example of nested VT decoder when $n=32$, $M=3$, $\ell=2$, $m=2$, and $d_{sec}=7$.\label{Fig:ex_nested_decoder}}
\end{figure}


\subsection{Nested VT decoder plus erasure decoder}
\label{subsect:VTdecoder_erasure_decoder}

As we discussed in Section~\ref{Section:erasure_nested}, when our nested VT decoder discovers multiple candidate combinations with length $n$ that satisfy all the VT conditions, it takes the overlap of these output sequences as the reconstructed sequence. This may result in some missing pieces, which can be viewed as erasures. We add an erasure code during encoding and  an erasure decoder to to handle these missing pieces.

% {\color{red} do you take the overlap of the reassembled sequences or the reconstructed data bits? I though it was the former, but your example is the latter.}

% \sncomment{We can take the overlap of either reassembled sequences or the reconstructed data bits because the nested VT code preserves the data structure. In particular, if we take the overlap of reassembled sequences, some of the parity bits will also be erased in addition to the erased data bits. But these erased parity bits won't change the data bits since, at the VT decoder, we don't use the parity bits to decode the data bits (we only use parity bits to find the reconstructed codewords (i.e., $\Pi_1$ and $\Pi_2$ in this example) that satisfy all VT conditions). }

For instance, in Fig.~\ref{Fig:ex_overlap}, the chop-and-shuffle channel breaks codeword $\textbf{x}=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~1~0~1~0~0~1~1~0~0$
$0~1~0~0~1~0~0~0~0]$ into $M=6$ different fragments, in which two fragments contain only one bit each. Here, if we use Algorithm~\ref{algo:decoder} to execute the nested VT decoder, we obtain two strings $\Pi_1=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~1~0~1~0~0~1~1~0~0~0~1~0~0~1~0~0~0~0]$ and $\Pi_2=[1~0~1~1~0~0~1~0~0~0~1~0~1~0~0~1~1~0~1~0~1~0~0~0~1~0~0~1$ $0~0~0~0]$, both of which meet all the VT conditions and removing the parity bits results in $\hat{\textbf{d}}_1=[1~0~1~1~0~0~1~1~0~1~0~1~0~0]$ and $\hat{\textbf{d}}_2=[1~0~1~1~0~0~1~1~0~0~1~1~0~1]$ as the decode data bits. This shows that short fragments lead to more than one decoded data sequences. Finally, we take the overlap between $\hat{\textbf{d}}_1$ and $\hat{\textbf{d}}_2$ and conclude that $\hat{\textbf{d}}=[1~0~1~1~0~0~1~1~0~E~E~1~0~E]$ is the recovered data bits where $E$ describes the erasures.

\begin{figure*}[h]
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.75\linewidth]{images/overlap_erasure_ex_r_0.png}
  \caption{\it An example of having more than one decoded data bits when $n=32$, $M=6$, $\ell=2$, $m=2$, and $d_{sec}=7$.\label{Fig:ex_overlap}}
\end{figure*}


==> sections/Section7_simulation_results.tex <==
This section provides the simulation results of our work that are done in MATLAB and available online at~\cite{key}. 

We assume input data bits $\textbf{d}$ is a random binary string wherein each element is an independently and identically distributed Bernoulli$(1/2)$ random variable. Moreover, we consider the length of $\textbf{d}$ to be $m^{(\ell-1)}d_{sec}$, and our nested encoder uses $\ell$ encoding layers. Then, we assume the chop-and-shuffle channel breaks codeword $\textbf{x}$ into $M$ different fragments where the length of each broken fragment is an independent random variable following a Geometric distribution with $p_n=\alpha/\log_2(n)$. Furthermore, we use an erasure code with a rate of $1-\epsilon$ before our nested VT encoder to indicate the role of missing fragments in our simulation, and $\epsilon$ is obtained heuristically. Moreover, the rate of our scheme equals to 
\begin{align}
    R_t=(1-\epsilon)R,
\end{align}
where $R$ is the rate of nested VT code. 

{\color{brown}We assume that our decoder performs decoding procedure in limited time $\Delta$ and an error occurs if the decoder attains $\hat{\textbf{d}}$ during $\Delta$, but $\hat{\textbf{d}}\neq\textbf{d}$. In Table~\ref{table:increase_Delta}, we compare the number of cases where the decoding algorithm cannot discover $\hat{\textbf{d}}$ within $\Delta$. It shows that these cases represent a small fraction of total cases and decrease as we increase the time.}

\begin{table}[h]
\caption{{\color{brown}The number of cases where our algorithm fails to find $\hat{\mathbf{d}}$ within $\Delta$ when $d_{sec}=185$, $m=3$, $\ell=3$, $n = 2016$, $\alpha=0.05$, $R_t=0.8194$, and $r_i^{(l)}=0$.}}
\centering
\begin{tabular}{|c|c|}
\hline

 & Number of cases where the decoder cannot get \\
 $\Delta~(\mathrm{sec})$ &   $\hat{\textbf{d}}$ within $\Delta$ / Total cases\\[0.5ex]
\hline \hline
10 & 0.014\\
50 & 0.007 \\
100 & 0.005\\
500 & 0.002\\ %[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:increase_Delta}
%\vspace{-5mm}
\end{table}


%for recovering the data-bit.
%an error occurs when the reconstructed data does not match the input data. %{\color{red} what does this last sentence mean? an error occurs when your reconstructed data does not match the input.}

%{\color{red} remind the reader what $R_t$ is.}

Fig.\ref{Fig:error_rates} depicts the error rate of our solution as a function of the codeword length $n$ on a logarithmic scale. Specifically, it includes three error rate curves when  $\alpha=0.05, 0.1$, and $0.2$ and $R_t$ is equal to $0.8194, 0.7535,$ and $0.6114$, respectively. As we see in Fig.\ref{Fig:error_rates}, the error rate decreases as the length of codeword increases, and this shows the decoding error decreases as $n$ grows. % {\color{red} can you quantify how the pace of decrease? is it polynomial, exponential, etc?}

% \sncomment{I used ``cftool'' in MATLAB and got Fig.~\ref{Fig:curve_fit}. It shows that the decoding error decreases exponentially when $\alpha=0.2$ ($\text{Error-rate}\approx0.1e^{-0.003n}$)}

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/curve_fitting.png}
  \caption{\it \sncomment{Curve fitting using cftool in MATLAB when $\alpha=0.2$.}\label{Fig:curve_fit}}
\end{figure}
\end{comment}

Note that we obtain $\epsilon$
heuristically such that $R_t=(1-\epsilon)R$ holds for all cases.
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/Fig_error_rates.eps}
  \caption{\it Error rates with different values of $\alpha$\label{Fig:error_rates}}
\end{figure}

Earlier we asked whether using either $r_i^{(l)}\neq 0$ or unique residues as $r_i^{(l)}=i-1$ for different VT codewords in each layer would benefit the results. To answer this, in Table~\ref{table:diff_r_methods}, we summarize the simulation results for different methods of selecting $r_i^{(l)}$ when $d_{sec}=185$, $m=3$, $\ell=3$, $n = 2016$, $\alpha=0.05$, $R_t=0.8194$, and $\Delta=20~\mathrm{sec}$.%{\color{red} Sajjad, is $t_{lim}$ the same as $\Delta_t$? If so, unify the notation. Also, I don't think you need the subscript in $\Delta_t$.}
According to Table~\ref{table:diff_r_methods}, using different residues for different VT codewords reduces the number of cases where the decoder does not obtain $\hat{\textbf{d}}$ during $\Delta$, but only slightly. However, it shows that using $r_i^{(l)} \neq 0$ degrades the error rate. In fact, \cite{sloane2002single} shows that there are more VT codewords with $r_i^{(l)} = 0$ than any other value for $r_i^{(l)}$. This means with higher values of $r_i^{(l)}$, the number of codewords decreases, and it might be the case that this increases the chance of different arrangements satisfying the VT conditions. 

%{\color{brown} According to Fig.~\ref{Fig:compare_error_rate_r_0_diff_r}, using different unique residues for different VT codewords improves the decoding error slightly, compared to using $r=0$ for all VT codewords. Furthermore, our simulations show that the complexity of both above methods is almost the same.}

% \begin{figure}
%     \centering
%     \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/compare_error_rate_r_0_uniq_res.png}
%   \caption{\it A comparison between having $r=0$ for all VT codewords and having a unique residue for each codeword as $r_i^{(l)}=i-1, 1 \leq l \leq \ell$ when $\alpha=0.05$ and $R_t=0.8194$.\label{Fig:compare_error_rate_r_0_diff_r}}
% \end{figure}

\begin{table}[h]
\caption{{\color{brown}Comparison between different methods of choosing $r_i^{(l)}$ when $d_{sec}=185$, $m=3$, $\ell=3$, $n = 2016$, $\alpha=0.05$, $R_t=0.8194$, and $\Delta=20~\mathrm{sec}.$}}
\centering
\begin{tabular}{|c|c|c|}
\hline

 & Number of cases that the decoder does not &\\
$r_i^{(l)}$ & attain $\hat{\textbf{d}}$ within $\Delta$/ Total cases & Error rate\\[0.5ex]

\hline \hline
Unique & 0.006 & 0.011 \\
0  & 0.008 & 0.011 \\
5  & 0.196 & 0.018\\
10 & 0.263 & 0.265\\
50 & 0.267 & 0.286\\ %[1ex]  % [1ex] adds vertical space
\hline
\end{tabular}
\label{table:diff_r_methods}
%\vspace{-5mm}
\end{table}


In Fig.~\ref{Fig:complexity}, we describe the complexity of our decoding scheme in terms of the number of permutations that our approach explores during the decoding process, and we use the brute-force search as the baseline. The brute-force solution goes through $M!$ cases, which grows approximately (Stirling's approximation) as $M^M$. %{\color{red} verify my changes} \sncomment{ $M!$ is faster than exponential function $a^M$ and slower than $M^M$. In other words, $\lim_{M\rightarrow \infty}\frac{a^M}{M!}=0$ and $\lim_{M\rightarrow \infty}\frac{M!}{M^M}=0$.} 
In Fig.~\ref{Fig:complexity},  we consider the complexity of our approach divided by $M!$ versus the codeword length in a logarithmic fashion. It indicates that our approach significantly reduces the complexity compared to the brute-force method.
\begin{figure}
    \centering
    \includegraphics[trim = 0mm 0mm 0mm 0mm, clip, scale=7, width=0.99\linewidth]{images/Fig_Complexity_r_0.eps}
  \caption{\it The complexity of our approach in terms of a number of cases that are searched through the decoding algorithm when $\alpha=0.05$, $\ell=3$, and $n \in (2^8,2^{14})$.\label{Fig:complexity}}
\end{figure}

==> sections/Section8_conclusion.tex <==
Motivated by recent advances in DNA-based storage, in this paper, we investigated the chop-and-shuffle channel that breaks the input sequence into a random number of variable-length fragments. We designed an encoding/decoding scheme based on a nested structure of Varshamov-Tenengolts (VT) codes to retrieve data bits from the non-overlapping fragments. We showed through simulations that our approach provides higher rates than the lower-bound in~\cite{TornPaperCoding}, and the decoding error decreases as the codeword length increases. Moreover, we proposed a new method with linear complexity to build a single VT code that requires fewer parity bits compared to~\cite{sloane2002single}.

==> sections/abstract.tex <==
We study the problem of retrieving data from a channel that breaks the input sequence into a set of unordered fragments of random lengths, which we refer to as the chop-and-shuffle channel. The length of each fragment follows a geometric distribution. We propose nested Varshamov-Tenengolts (VT) codes to recover the data. We evaluate the error rate and the complexity of our scheme numerically. Our results show that the decoding error decreases as the input length increases, and our method has a significantly lower complexity than the baseline brute-force approach. We also propose a new construction for VT codes, quantify the maximum number of the required parity bits, and show that our approach requires fewer parity bits compared to known results.
